Video Analytics with Zero-streaming Cameras

Low-cost cameras enable powerful analytics. An unexploited opportunity is that most captured videos remain "cold" without being queried. For efficiency, we advocate for these cameras to be zero streaming: capturing videos to local storage and communicating with the cloud only when analytics is requested. How to query zero-streaming cameras efficiently? Our response is a camera/cloud runtime system called DIVA. It addresses two key challenges: to best use limited camera resource during video capture; to rapidly explore massive videos during query execution. DIVA contributes two unconventional techniques. (1) When capturing videos, a camera builds sparse yet accurate landmark frames, from which it learns reliable knowledge for accelerating future queries. (2) When executing a query, a camera processes frames in multiple passes with increasingly more expensive operators. As such, DIVA presents and keeps refining inexact query results throughout the query's execution. On diverse queries over 15 videos lasting 720 hours in total, DIVA runs at more than 100x video realtime and outperforms competitive alternative designs. To our knowledge, DIVA is the first system for querying large videos stored on low-cost remote cameras.

==> eval-adapt.tex <==
% !TeX root = main.tex
%\subsection{Adapting to Environmental Variants}
%\subsection{Adaptation of query plan to resources}
\subsection{Adaptation to hardware resources}
\label{sec:eval:adapt}
%\label{eval-adapt}
\input{fig-adapt}

\sys{} benefits from its adaptive selection of on-camera operators. 
%\st{\textit{default setup} is running with 1MB/s network on Raspberry Pi 3.
%Then we change the network to 2MB/s and 0.5MB/s, and also the camera hardware to odroid independently to see how \sys{} performs.}
To demonstrate so, we test \sys{}'s performance on several camera/network resource configurations and compare it to fixing the operators to be the ones picked by \sys{} with the default resources.
As shown in Figure~\ref{fig:eval-adapt}, the adaptation speeds up \textit{retrieval} and \textit{tagging} queries by up to 37\% and 30\%, respectively.
%Take Figure~\ref{fig:eval-adapt}(a) as an example:
We observe that under \textit{higher} network bandwidth (2 MB/s), \sys{} automatically picks a series of faster operators, starting from one having one less convolutional layer and 2$\times$ smaller kernel;
%(one key aspect of operator upgrade in \S\ref{sec:overview}).
on a \textit{faster} camera (Odroid), \sys{} picks a series of slower operators, starting from one with one extra convolutional layer and 2$\times$ more parameters in dense layers. 

% -- too generic ! --
\begin{comment}
under higher network bandwidth (2 MB/s), \sys{} automatically picks a series of faster operators to match the bandwidth, one key aspect of operator upgrade (\S\ref{sec:overview}).
In the retrieval case, the initial operator has one less convolutional layer and 2X reduction in fully-connected layer size.
Running on the faster camera (Odroid) than the default one (Rpi3), \sys{} automatically picks heavier (more accurate) operators as they run fast enough to match the network speed. 
\end{comment}

% --- verbose --- 
%First, \sys{}, with or without adaptation, consistently outperforms other baselines under variant configurations.
%More specifically, XYZ is 11.4$\times$ $\sim$ 14.2$\times$ better than cloud-only approach, while Cam-Focus and Cam-NoScope are only up to 2.4$\times$ and 4.1$\times$, respectively.
%Similarly in tagging query, XYZ is 23.1$\times$ $\sim$ 29.7$\times$ faster than cloud-only approach, while Cam-Focus and Cam-NoScope are no better than 5.3$\times$ and 5.9$\times$, respectively.
%When running on odroid, \sys{} and Cam-NoScope exhibit better performance as odroid is relatively more powerful than raspberry pi, which means that the operators can run faster.



% \item \textbf{user-specified error tolerance}
% How sensitive we are towards error tolerance? If the error tolerance is higher, e.g., 5\%, we can definitely tag a lot faster. Improtant: we can still beat NoScope and Focus, but how much is the improvement?


==> eval-scale.tex <==
% !TeX root = main.tex
\subsection{System Scalability}\label{eval-scale}

how many ongoing queries can be supported on one GPU (before the CPU saturates)

\textbf{Our system can scale up for more videos with more GPUs}

will training become bottleneck?

make some estimation, how much money we have burned?

==> eval-videos.tex <==
% !TeX root = main.tex

This also accounts for \sys{}'s varying (yet substantial) advantages over the alternatives observed in end-to-end results. 
As examples, 
for retrieval (Figure~\ref{fig:perf-combine}(a)): \sys{}'s advantages are more pronounced on chaweng than on banff; 
for tagging (Figure~\ref{fig:perf-combine}(b)): the advantages are more pronounced on jackson\_h than on mierlo;
for counting (Figure~\ref{fig:counting}): they are more pronounced on whitebay than on venice. 
Indeed, we observe such skewness exists widely across most videos.


\begin{comment}
\noindent \textbf{Performance sensitivity to video contents}
Across different videos, \sys{} sees substantial, yet varying advantages over the alternatives.
For example, \sys{} brings more retrieval improvements on \textit{chaweng} (Figure~\ref{fig:retrieval-perf}(c)) than \textit{banff} (Figure~\ref{fig:retrieval-perf}(f)).
% For example, to retrieve 99\% instances, \sys{} performs much better on \textit{chaweng} video, i.e., 10$\times$ and 8$\times$ lower latency than \focus{} and \noscope{}, respectively.
% While on \textit{banff} video, the improvements by \sys{} is smaller (3.5$\times$ and 2.3$\times$).
The similar observations can also be made from tagging (\textit{jackson\_h} vs. \textit{mierlo}) and counting (\textit{whitebay} vs. \textit{venice}) queries.
The main reason is that \textit{chaweng} video has better spatial locality exploit, as the object (bicycle) only appears at 1/8 region, while for \textit{banff} video the object (bus) appears at 4/5 region.
As described previously, spatial locality helps to further specialize and optimize the performance of each single operator.

Note that, though, even on videos like banff, the improvements of \sys{} are still significant enough since our operator upgrade technique doesn't rely on such video characteristic.

%\note{counting}
%%\paragraph{Performance across videos}
%The end-to-end performance varies across different videos.
%The object in whitebay \note{persons} is much larger than venice, and the frames are not captured from high-angle cameras, so that our ranker NNs work better on whitebay than on venice, and end up with shorter end-to-end time to return the max number of object.
%\note{this is comparing across videos? less interesting}
%
%\note{tagging}
%%\noindent \textbf{Performance across videos}
%Similar to retrieval, the tagging performance of \sys{} is diverse across different videos.
%For example, \sys{} performs much better on jackson\_h video, i.e., 5$\times$ and 12$\times$ lower latency than Cam-Focus and Cam-NoScope, respectively.
%While on venice video, the improvements by \sys{} is smaller.
%\note{what's the reason?}
\end{comment}


==> evidence.tex <==

\mwx{The new evidence below. Note: they are not wireless; it's affected by coronavirus.}

\paragraph{A campus case of cold videos}
As supporting evidence, we collected video query data from a campus the authors affiliated with.
Occupying around 2 km$^2$ area, the campus is equipped with more than 1,800 (950) outdoor (indoor) surveillance cameras.
Currently, all captured videos are streamed to an edge server, stored for 2--3 months, and queried retrospectively.
The queries are mostly ML-based, e.g., object detection or license plate recognition, but also support manual inspection.
During the 2-months data collection period, only 3 queries are executed that span 0.65\% cameras and 0.0018\% video data generated.
Based on the collected data, we estimate that more than 99.9\% videos remain cold and will never be queried.


==> fig-adapt.tex <==
% !TeX root = main.tex
\begin{figure}[t]
	\centering
		\includegraphics[width=.45\textwidth]{figs/eval/adapt/adapt.pdf}

	\caption{\textbf{\sys{}'s adaptation brings a noticeable performance benefit}. 
	% Query performance (x-axis) under different upload bandwidth / camera hardware (y-axis). 
	% Performance normalized to \cloudonly{} under respective resources. 
	(a) Average performance on \textit{retrieving} 50\%/80\%/99\% instances on \chaweng{}/\oxford{}.
	(b) Average performance on \textit{tagging} one in every 10/3/1 frames on \jacksont{}/\boathouse{}.
	\sys{} even w/o adaptation outperforms the alternatives significantly.
	}
	\label{fig:eval-adapt}
	\vspace{-10pt}
\end{figure}



%When the landmarks are very dense (>= 1/10FPS), we don't exhausively send all the landmarks (which could be slow) but send frames just enough to make the model converge at bootstrap stage. 

==> fig-counting-avg.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering					
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/counting-avg/whitebay-avg.png}
		\subcaption{whitebay -- person}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/counting-avg/venice-avg.png}
		\subcaption{venice -- person}
	\end{minipage}


	\centering					
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/counting-avg/shibuya-avg.png}
		\subcaption{shibuya -- car}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.24\textwidth}
		\includegraphics[width=1\textwidth]{figs/counting-avg/banff-avg.png}
		\subcaption{banff -- car}
	\end{minipage}
	
	\caption{Average Counting}
	\label{fig:counting-avg}
\end{figure}

==> fig-crop-nn.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.48\textwidth]{figs/crop-nn.jpg}

	\caption{NN on cropped regions}
	\label{fig:retrieval-multi}
\end{figure}

==> fig-e2e-perf.tex <==
% !TeX root = main.tex
\begin{figure*}
	\centering
	\includegraphics[width=0.98\textwidth]{figs/e2e-perf.jpg}
	\caption{End-to-end performance (can add multiple lines/bars in above graph for different objects)}
	\label{fig:retrieval-multi}
\end{figure*}

==> fig-exec.tex <==
% !TeX root = main.tex

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{figs/exec}
	%\vspace*{-.6cm}
	\caption{\textbf{According to a query's type, \sys{} executes (a) rankers or (b) filters on cameras}.}
	\label{fig:exec}
	\vspace{-8pt}
\end{figure}



==> fig-hm-objects.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.49\textwidth]{figs/heatmap/heatmap-objects.pdf}

	\caption{
	Of the same video, object classes may exhibit different spatial distribution. \textbf{XXX Car->Cars, Person->Persons}. Video length: XX hours each; see Table~\ref{tab:videos} for details. 
 	}
	\label{fig:hm-objects}
\end{figure}

==> fig-hm-videos.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{figs/heatmap/heatmap-video.pdf}
	\caption{In surveillance videos, object distribution exhibits spatial skewness. \textbf{XXX Car->Cars, Person->Persons}. Video length: XX hours each. See Table~\ref{tab:videos} for video details.}
	\label{fig:hm-video}
\end{figure}

==> fig-retrieval-perf.tex <==
% !TeX root = main.tex
% \begin{figure}
% 	\centering					
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/ashland.pdf}
% 		% \subcaption{ashland}
% 	\end{minipage}	
% 	% ~
% 	% \begin{minipage}[b]{0.24\textwidth}
% 	% 	\includegraphics[width=1\textwidth]{figs/eval/retrieval/banff.pdf}
% 	% 	\subcaption{banff}
% 	% \end{minipage}	
% 	~
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/boathouse.pdf}
% 		% \subcaption{boathouse}
% 	\end{minipage}	

% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/chaweng.pdf}
% 		% \subcaption{chaweng}
% 	\end{minipage}	
% 	% ~
% 	% \centering					
% 	% \begin{minipage}[b]{0.24\textwidth}
% 	% 	\includegraphics[width=1\textwidth]{figs/eval/retrieval/shibuya-park.pdf}
% 	% 	\subcaption{shibuya\_p}
% 	% \end{minipage}
% 	~			
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/oxford.pdf}
% 		% \subcaption{oxford}
% 	\end{minipage}

% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/shibuya-park.pdf}
% 		% \subcaption{shibuya\_p}
% 	\end{minipage}
% 	~			
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/retrieval/banff.pdf}
% 		% \subcaption{banff}
% 	\end{minipage}
	

	
% 	\caption{Retrieval performance acorss different videos. All lines are cut at 99\%. Red triangles indicate when operators are upgraded. \textbf{XXX 48 hour videos}}
% 	\label{fig:retrieval-perf}
% \end{figure}

\begin{figure}
	\centering					
	\includegraphics[width=.48\textwidth]{figs/eval/retrieval/retrieval-perf.pdf}
	\caption{For \textit{retrieval} queries, \sys{} shows good performance and outperforms the alternatives. 
	Each query covers a 48-hour video. 
%	All lines are cut at 99\%. 
	Red triangles: \sys{} upgrading operators}
	\label{fig:retrieval-perf}
\end{figure}

==> fig-tagging-perf.tex <==
% !TeX root = main.tex
\begin{figure}
	\centering					
	\includegraphics[width=.48\textwidth]{figs/eval/tagging/tagging-perf.pdf}

	
	\caption{For \textit{tagging} queries, \sys{} shows good performance and outperforms the alternatives. 
	Each query covers a 48-hour video. 
%	All lines are cut at 99\%. 
	Red triangles: \sys{} upgrading operators}
	\label{fig:tagging-perf}
\end{figure}

% \begin{figure}
% 	\centering					
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/eagle.pdf}
% 		% \subcaption{eagle}
% 	\end{minipage}	
% 	~
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/coral-reef.pdf}
% 		% \subcaption{coral-reef}
% 	\end{minipage}	

	
% 	\centering
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/jackson_t.pdf}
% 		% \subcaption{jackson\_t}
% 	\end{minipage}
% 	~
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/jackson_h.pdf}
% 		% \subcaption{jackson\_h}
% 	\end{minipage}

% 	\centering
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/mierlo.pdf}
% 		% \subcaption{mierlo}
% 	\end{minipage}
% 	~
% 	\begin{minipage}[b]{0.24\textwidth}
% 		\includegraphics[width=1\textwidth]{figs/eval/tagging/lausanne.pdf}
% 		% \subcaption{lausanne}
% 	\end{minipage}

	
% 	\caption{Tagging performance across different videos.}
% 	\label{fig:tagging-perf}
% \end{figure}

==> figs/eval/adapt/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> figs/eval/local/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> figs/heatmap/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> figs/op-spd-acc/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> figs/pdfcrop <==
#!/usr/bin/env perl
use strict;
$^W=1; # turn warning on
#
# pdfcrop.pl
#
# Copyright (C) 2002, 2004, 2005, 2008-2012 Heiko Oberdiek.
#
# This program may be distributed and/or modified under the
# conditions of the LaTeX Project Public License, either version 1.2
# of this license or (at your option) any later version.
# The latest version of this license is in
#   http://www.latex-project.org/lppl.txt
# and version 1.2 or later is part of all distributions of LaTeX
# version 1999/12/01 or later.
#
# See file "README" for a list of files that belong to this project.
#
# This file "pdfcrop.pl" may be renamed to "pdfcrop"
# for installation purposes.
#
my $prj         = 'pdfcrop';
my $file        = "$prj.pl";
my $program     = uc($&) if $file =~ /^\w+/;
my $version     = "1.38";
my $date        = "2012/11/02";
my $author      = "Heiko Oberdiek";
my $copyright   = "Copyright (c) 2002-2012 by $author.";
#
# Reqirements: Perl5, Ghostscript
# History:
#   2002/10/30 v1.0:  First release.
#   2002/10/30 v1.1:  Option --hires added.
#   2002/11/04 v1.2:  "nul" instead of "/dev/null" for windows.
#   2002/11/23 v1.3:  Use of File::Spec module's "devnull" call.
#   2002/11/29 v1.4:  Option --papersize added.
#   2004/06/24 v1.5:  Clear map file entries so that pdfTeX
#                     does not touch the fonts.
#   2004/06/26 v1.6:  Use mgs.exe instead of gswin32c.exe for MIKTEX.
#   2005/03/11 v1.7:  Support of spaces in file names
#                     (open("-|") is used for ghostscript call).
#   2008/01/09 v1.8:  Fix for moving the temporary file to the output
#                     file across file system boundaries.
#   2008/04/05 v1.9:  Options --resolution and --bbox added.
#   2008/07/16 v1.10: Support for XeTeX added with new options
#                     --pdftex, --xetex, and --xetexcmd.
#   2008/07/22 v1.11: Workaround for open("-|").
#   2008/07/23 v1.12: Workarounds for the workaround (error detection, ...).
#   2008/07/24 v1.13: open("-|")/workaround removed.
#                     Input files with unsafe file names are linked/copied
#                     to temporary file with safe file name.
#   2008/09/12 v1.14: Error detection for invalid Bounding Boxes.
#   2009/07/14 v1.15: Fix for negative coordinates in Bounding Boxes
#                     (David Menestrina).
#   2009/07/16 v1.16: Security fixes:
#                     * -dSAFER added for Ghostscript,
#                     * -no-shell-escape added for pdfTeX/XeTeX.
#   2009/07/17 v1.17: Security fixes:
#                     * Backticks and whitespace are forbidden
#                       for options --(gs|pdftex|xetex)cmd.
#                     * Validation of options --papersize and --resolution.
#   2009/07/18 v1.18: * Restricted mode added.
#                     * Option --version added.
#   2009/09/24 v1.19: * Ghostscript detection rewritten.
#                     * Cygwin: `gs' is preferred to `gswin32c'.
#   2009/10/06 v1.20: * File name sanitizing in .tex file.
#   2009/12/21 v1.21: * Option --ini added for IniTeX mode.
#                     * Option --luatex and --luatexcmd added for LuaTeX.
#   2009/12/29 v1.22: * Syntax description for option --bbox fixed
#                       (Lukas Prochazka).
#   2010/01/09 v1.23: * Options --bbox-odd and -bbox-even added.
#   2010/08/16 v1.24: * Workaround added for buggy ghostscript ports
#                       that print the BoundingBox data twice.
#   2010/08/26 v1.25: * Fix for the case that the PDF file contains
#                       an entry /CropBox different to /MediaBox.
#                     * \pageinclude implemented for XeTeX.
#                     * XeTeX: --clip does not die, but this option
#                       is ignored, because XeTeX always clip.
# 2010/08/26 v1.26: * XeTeX's \XeTeXpdffile expects keyword
#                     `media', not `mediabox'.
#                   * New option --pdfversion.
#                     Default is `auto' that means the PDF version
#                     is inherited from the input file. Before
#                     pdfcrop has used the TeX engine's default.
#                   * Option --luatex fixed (extra empty page at end).
# 2010/09/03 v1.27: * Workaround of v1.24 fixed.
# 2010/09/06 v1.28: * The Windows registry is searched if Ghostscript
#                     is not found via PATH.
#                   * Windows only: support of spaces in command
#                     names in unrestricted mode.
# 2010/09/06 v1.29: * Find the latest Ghostscript version in registry.
# 2010/09/15 v1.30: * Warning of pdfTeX because of \pdfobjcompresslevel
#                     avoided when reducing \pdfminorversion.
#                   * Fix for TeX syntax characters in input file names.
# 2010/09/17 v1.31: * Passing the input file name via hex string to TeX.
#                   * Again input file names restricted for Ghostscript
#                     command line, switch then to symbol link/copy
#                     method.
# 2011/08/10 v1.32: * Detection for gswin64c.exe added.
# 2012/02/01 v1.33: * Input file can be `-' (standard input).
# 2012/04/18 v1.34: * Format of --version changed
#                     from naked version number to a line with
#                     program name, date and version.
# 2012/10/15 v1.35: * Additional debug infos added for Perl version.
# 2012/10/16 v1.36: * More error codes added.
# 2012/10/16 v1.37: * Extended error messages if available.
#                   * Fix for broken v1.36.
# 2012/11/02 v1.38: * Fix for unsufficient cleanup, if function `cleanup' is
#                     prematurely called in `eval' for `symlink' checking.

### program identification
my $title = "$program $version, $date - $copyright\n";

### error strings
my $Error = "!!! Error:"; # error prefix

### make ENV safer
delete @ENV{qw(IFS CDPATH ENV BASH_ENV)};

# Windows detection (no SIGHUP)
my $Win = 0;
$Win = 1 if $^O =~ /mswin32/i;
$Win = 1 if $^O =~ /cygwin/i;
use Config;
my $archname = $Config{'archname'};
$archname = 'unknown' unless defined $Config{'archname'};

### extended error messages
sub exterr () {
    chomp(my $msg_errno = $!);
    chomp(my $msg_extended_os_error = $^E);
    if ($msg_errno eq $msg_extended_os_error) {
        $msg_errno;
    }
    else {
        "$msg_errno/$msg_extended_os_error";
    }
}

### string constants for Ghostscript run
# get Ghostscript command name
$::opt_gscmd = '';
sub find_ghostscript () {
    return if $::opt_gscmd;
    if ($::opt_debug) {
        print "* Perl executable: $^X\n";
        if ($] < 5.006) {
            print "* Perl version: $]\n";
        }
        else {
            printf "* Perl version: v%vd\n", $^V;
        }
        if (defined &ActivePerl::BUILD) {
            printf "* Perl product: ActivePerl, build %s\n", ActivePerl::BUILD();
        }
        use Config;
        printf "* Pointer size: $Config{'ptrsize'}\n";
        printf "* Pipe support: %s\n",
                (defined($Config{'d_pipe'}) ? 'yes' : 'no');
        printf "* Fork support: %s\n",
                (defined($Config{'d_fork'}) ? 'yes' : 'no');
    }
    my $system = 'unix';
    $system = "dos" if $^O =~ /dos/i;
    $system = "os2" if $^O =~ /os2/i;
    $system = "win" if $^O =~ /mswin32/i;
    $system = "cygwin" if $^O =~ /cygwin/i;
    $system = "miktex" if defined($ENV{"TEXSYSTEM"}) and
                          $ENV{"TEXSYSTEM"} =~ /miktex/i;
    print "* OS name: $^O\n" if $::opt_debug;
    print "* Arch name: $archname\n" if $::opt_debug;
    print "* System: $system\n" if $::opt_debug;
    my %candidates = (
        'unix' => [qw|gs gsc|],
        'dos' => [qw|gs386 gs|],
        'os2' => [qw|gsos2 gs|],
        'win' => [qw|gswin32c gs|],
        'cygwin' => [qw|gs gswin32c|],
        'miktex' => [qw|mgs gswin32c gs|]
    );
    if ($system eq 'win' or $system eq 'cygwin' or $system eq 'miktex') {
        if ($archname =~ /mswin32-x64/i) {
            my @a = ();
            foreach my $name (@{$candidates{$system}}) {
                push @a, 'gswin64c' if $name eq 'gswin32c';
                push @a, $name;
            }
            $candidates{$system} = \@a;
        }
    }
    my %ext = (
        'unix' => '',
        'dos' => '.exe',
        'os2' => '.exe',
        'win' => '.exe',
        'cygwin' => '.exe',
        'miktex' => '.exe'
    );
    my $candidates_ref = $candidates{$system};
    my $ext = $Config{'_exe'};
    $ext = $ext{$system} unless defined $ext;
    use File::Spec;
    my @path = File::Spec->path();
    my $found = 0;
    foreach my $candidate (@$candidates_ref) {
        foreach my $dir (@path) {
            my $file = File::Spec->catfile($dir, "$candidate$ext");
            if (-x $file) {
                $::opt_gscmd = $candidate;
                $found = 1;
                print "* Found ($candidate): $file\n" if $::opt_debug;
                last;
            }
            print "* Not found ($candidate): $file\n" if $::opt_debug;
        }
        last if $found;
    }
    if (not $found and $Win) {
        $found = SearchRegistry();
    }
    if ($found) {
        print "* Autodetected ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
    else {
        $::opt_gscmd = $$candidates_ref[0];
        print "* Default ghostscript command: $::opt_gscmd\n" if $::opt_debug;
    }
}

sub SearchRegistry () {
    my $found = 0;
    eval 'use Win32::TieRegistry qw|KEY_READ REG_SZ|;';
    if ($@) {
        if ($::opt_debug) {
            print "* Registry lookup for Ghostscript failed:\n";
            my $msg = $@;
            $msg =~ s/\s+$//;
            foreach (split /\r?\n/, $msg) {
                print "  $_\n";
            }
        }
        return $found;
    }
    my $open_params = {Access => KEY_READ(), Delimiter => '/'};
    my $key_name_software = 'HKEY_LOCAL_MACHINE/SOFTWARE/';
    my $current_key = $key_name_software;
    my $software = new Win32::TieRegistry $current_key, $open_params;
    if (not $software) {
        print "* Cannot find or access registry key `$current_key'!\n"
                if $::opt_verbose;
        return $found;
    }
    print "* Search registry at `$current_key'.\n" if $::opt_debug;
    my %list;
    foreach my $key_name_gs (grep /Ghostscript/i, $software->SubKeyNames()) {
        $current_key = "$key_name_software$key_name_gs/";
        print "* Registry entry found: $current_key\n" if $::opt_debug;
        my $key_gs = $software->Open($key_name_gs, $open_params);
        if (not $key_gs) {
            print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
            next;
        }
        foreach my $key_name_version ($key_gs->SubKeyNames()) {
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            print "* Registry entry found: $current_key\n" if $::opt_debug;
            if (not $key_name_version =~ /^(\d+)\.(\d+)$/) {
                print "  The sub key is not a version number!\n" if $::opt_debug;
                next;
            }
            my $version_main = $1;
            my $version_sub = $2;
            $current_key = "$key_name_software$key_name_gs/$key_name_version/";
            my $key_version = $key_gs->Open($key_name_version, $open_params);
            if (not $key_version) {
                print "* Cannot open registry key `$current_key'!\n" if $::opt_debug;
                next;
            }
            $key_version->FixSzNulls(1);
            my ($value, $type) = $key_version->GetValue('GS_DLL');
            if ($value and $type == REG_SZ()) {
                print "  GS_DLL = $value\n" if $::opt_debug;
                $value =~ s|([\\/])([^\\/]+\.dll)$|$1gswin32c.exe|i;
                my $value64 = $value;
                $value64 =~ s/gswin32c\.exe$/gswin64c.exe/;
                if ($archname =~ /mswin32-x64/i and -f $value64) {
                    $value = $value64;
                }
                if (-f $value) {
                    print "  EXE found: $value\n" if $::opt_debug;
                }
                else {
                    print "  EXE not found!\n" if $::opt_debug;
                    next;
                }
                my $sortkey = sprintf '%02d.%03d %s',
                        $version_main, $version_sub, $key_name_gs;
                $list{$sortkey} = $value;
            }
            else {
                print "  Missing key `GS_DLL' with type `REG_SZ'!\n" if $::opt_debug;
            }
        }
    }
    foreach my $entry (reverse sort keys %list) {
        $::opt_gscmd = $list{$entry};
        print "* Found (via registry): $::opt_gscmd\n" if $::opt_debug;
        $found = 1;
        last;
    }
    return $found;
}

# restricted mode
my $restricted = 0;
if ($0 =~ /rpdfcrop/ or $0 =~ /restricted/) {
    $restricted = 1;
}

# "null" device
use File::Spec::Functions qw(devnull);
my $null = devnull();

### variables
my $inputfile   = "";
my $outputfile  = "";
my $tmp = "tmp-\L$program\E-$$";

### paper sizes

my @papersizes = qw[
  11x17 ledger legal letter lettersmall
  archE archD archC archB archA
  a0 a1 a2 a3 a4 a4small a5 a6 a7 a8 a9 a10
  isob0 isob1 isob2 isob3 isob4 isob5 isob6
  c0 c1 c2 c3 c4 c5 c6
  jisb0 jisb1 jisb2 jisb3 jisb4 jisb5 jisb6
  b0 b1 b2 b3 b4 b5
  flsa flse halfletter
];
my %papersizes;
foreach (@papersizes) {
    $papersizes{$_} = 1;
}

### option variables
my @bool = ("false", "true");
$::opt_version    = 0;
$::opt_help       = 0;
$::opt_debug      = 0;
$::opt_verbose    = 0;
$::opt_pdftexcmd  = "pdftex";
$::opt_xetexcmd   = "xetex";
$::opt_luatexcmd  = "luatex";
$::opt_tex        = "pdftex";
$::opt_margins    = "0 0 0 0";
$::opt_clip       = 0;
$::opt_hires      = 0;
$::opt_papersize  = "";
$::opt_resolution = "";
$::opt_bbox       = "";
$::opt_bbox_odd   = "";
$::opt_bbox_even  = "";
$::opt_initex     = 0;
$::opt_pdfversion = "auto";

sub usage ($) {
    my $ret = shift;
    find_ghostscript();
    my $usage = <<"END_OF_USAGE";
${title}Syntax:   \L$program\E [options] <input[.pdf]> [output file]
Function: Margins are calculated and removed for each page in the file.
Options:                                                       (defaults:)
  --help              print usage
  --version           print version number
  --(no)verbose       verbose printing                         ($bool[$::opt_verbose])
  --(no)debug         debug informations                       ($bool[$::opt_debug])
  --gscmd <name>      call of ghostscript                      ($::opt_gscmd)
  --pdftex | --xetex | --luatex
                      use pdfTeX | use XeTeX | use LuaTeX      ($::opt_tex)
  --pdftexcmd <name>  call of pdfTeX                           ($::opt_pdftexcmd)
  --xetexcmd <name>   call of XeTeX                            ($::opt_xetexcmd)
  --luatexcmd <name>  call of LuaTeX                           ($::opt_luatexcmd)
  --margins "<left> <top> <right> <bottom>"                    ($::opt_margins)
                      add extra margins, unit is bp. If only one number is
                      given, then it is used for all margins, in the case
                      of two numbers they are also used for right and bottom.
  --(no)clip          clipping support, if margins are set     ($bool[$::opt_clip])
                      (not available for --xetex)
  --(no)hires         using `%%HiResBoundingBox'               ($bool[$::opt_hires])
                      instead of `%%BoundingBox'
  --(no)ini           use iniTeX variant of the TeX compiler   ($bool[$::opt_initex])
Expert options:
  --restricted        turn on restricted mode                  ($bool[$restricted])
  --papersize <foo>   parameter for gs's -sPAPERSIZE=<foo>,
                      use only with older gs versions <7.32    ($::opt_papersize)
  --resolution <xres>x<yres>                                   ($::opt_resolution)
  --resolution <res>  pass argument to ghostscript's option -r
                      Example: --resolution 72
  --bbox "<left> <bottom> <right> <top>"                       ($::opt_bbox)
                      override bounding box found by ghostscript
                      with origin at the lower left corner
  --bbox-odd          Same as --bbox, but for odd pages only   ($::opt_bbox_odd)
  --bbox-even         Same as --bbox, but for even pages only  ($::opt_bbox_even)
  --pdfversion <1.x> | auto | none
                      Set the PDF version to 1.x, 1 < x < 8.
                      If `auto' is given as value, then the
                      PDF version is taken from the header
                      of the input PDF file.
                      An empty value or `none' uses the
                      default of the TeX engine.               ($::opt_pdfversion)

Input file: If the name is `-', then the standard input is used and
  the output file name must be explicitly given.
Examples:
  \L$program\E --margins 10 input.pdf output.pdf
  \L$program\E --margins '5 10 5 20' --clip input.pdf output.pdf
In case of errors:
  Try option --verbose first to get more information.
In case of bugs:
  Please, use option --debug for bug reports.
END_OF_USAGE
    if ($ret) {
        die $usage;
    }
    else {
        print $usage;
        exit(0);
    }
}

### process options
my @OrgArgv = @ARGV;
use Getopt::Long;
GetOptions(
  "help!",
  "version!",
  "debug!",
  "verbose!",
  "gscmd=s",
  "pdftexcmd=s",
  "xetexcmd=s",
  "luatexcmd=s",
  "pdftex" => sub { $::opt_tex = 'pdftex'; },
  "xetex"  => sub { $::opt_tex = 'xetex'; },
  "luatex" => sub { $::opt_tex = 'luatex'; },
  "initex!",
  "margins=s",
  "clip!",
  "hires!",
  "papersize=s",
  "resolution=s",
  "bbox=s",
  "bbox-odd=s" => \$::opt_bbox_odd,
  "bbox-even=s" => \$::opt_bbox_even,
  "restricted" => sub { $restricted = 1; },
  "pdfversion=s" => \$::opt_pdfversion,
) or usage(1);
!$::opt_help or usage(0);

if ($::opt_version) {
    print "$prj $date v$version\n";
    exit(0);
}

$::opt_verbose = 1 if $::opt_debug;

@ARGV >= 1 or usage(1);

print $title;

print "* Restricted mode: ", ($restricted ? "enabled" : "disabled"), "\n"
        if $::opt_debug;

$::opt_pdfversion =~ /^(|none|auto|1\.([2-7]))$/
        or die "!!! Error: Invalid value `$::opt_pdfversion' for option `--pdfversion'!\n";
print "* Option `pdfversion': $::opt_pdfversion\n" if $::opt_debug;
$::opt_pdfversion = $2 if $2;
$::opt_pdfversion = '' if $::opt_pdfversion eq 'none';

find_ghostscript();

if ($::opt_bbox) {
    $::opt_bbox =~ s/^\s+//;
    $::opt_bbox =~ s/\s+$//;
    $::opt_bbox =~ s/\s+/ /;
    if ($::opt_bbox =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box: $::opt_bbox\n" if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox \"$::opt_bbox\")!\n";
    }
}
if ($::opt_bbox_odd) {
    $::opt_bbox_odd =~ s/^\s+//;
    $::opt_bbox_odd =~ s/\s+$//;
    $::opt_bbox_odd =~ s/\s+/ /;
    if ($::opt_bbox_odd =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for odd pages: $::opt_bbox_odd\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-odd \"$::opt_bbox_odd\")!\n";
    }
}
if ($::opt_bbox_even) {
    $::opt_bbox_even =~ s/^\s+//;
    $::opt_bbox_even =~ s/\s+$//;
    $::opt_bbox_even =~ s/\s+/ /;
    if ($::opt_bbox_even =~ /^-?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+ -?\d*\.?\d+$/) {
        print "* Explicite Bounding Box for even pages: $::opt_bbox_even\n"
                if $::opt_debug;
    }
    else {
        die "$Error Parse error (option --bbox-even \"$::opt_bbox_even\")!\n";
    }
}

@ARGV <= 2 or die "$Error Too many files!\n";

### input file
$inputfile = shift @ARGV;

if ($inputfile eq '-') {
    @ARGV == 1 or die "$Error Missing output file name!\n";
    print "* Input file: <stdin>\n" if $::opt_debug;
}
else {
    if (! -f $inputfile) {
        if (-f "$inputfile.pdf") {
            $inputfile .= ".pdf";
        }
        else {
            die "$Error Input file `$inputfile' not found!\n";
        }
    }
    print "* Input file: $inputfile\n" if $::opt_debug;
}

### output file
if (@ARGV) {
    $outputfile = shift @ARGV;
}
else {
    $outputfile = $inputfile;
    $outputfile =~ s/\.pdf$//i;
    $outputfile .= "-crop.pdf";
}

print "* Output file: $outputfile\n" if $::opt_debug;

### margins
my ($llx, $lly, $urx, $ury) = (0, 0, 0, 0);
if ($::opt_margins =~
        /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
    ($llx, $lly, $urx, $ury) = ($1, $2, $3, $4);
}
else {
    if ($::opt_margins =~ /^\s*([\-\.\d]+)\s+([\-\.\d]+)\s*$/) {
        ($llx, $lly, $urx, $ury) = ($1, $2, $1, $2);
    }
    else {
        if ($::opt_margins =~ /^\s*([\-\.\d]+)\s*$/) {
            ($llx, $lly, $urx, $ury) = ($1, $1, $1, $1);
        }
        else {
            die "$Error Parse error (option --margins)!\n";
        }
    }
}
print "* Margins: $llx $lly $urx $ury\n" if $::opt_debug;

### papersize validation (security)
if ($::opt_papersize ne '') {
    $::opt_papersize =~ /^[0-9A-Za-z]+$/
            or die "$Error Invalid papersize ($::opt_papersize)!\n";
    $papersizes{$::opt_papersize}
            or die "$Error Unknown papersize ($::opt_papersize),"
                   . " see ghostscript's documentation for option `-r'!\n";
}

### resolution validation (security)
if ($::opt_resolution ne '') {
    $::opt_resolution =~ /^\d+(x\d+)?$/
            or die "$Error Invalid resolution ($::opt_resolution),"
                   . " see ghostscript's documentation!\n";
}

### command name validation (security)
my %cmd = (
    'gscmd' => \$::opt_gscmd,
    'pdftexcmd' => \$::opt_pdftexcmd,
    'luatexcmd' => \$::opt_luatexcmd,
    'xetexcmd' => \$::opt_xetexcmd
);
foreach my $cmd (keys %cmd) {
    my $cmd_ref = $cmd{$cmd};
    $$cmd_ref =~ s/^\s+//;
    $$cmd_ref =~ s/\s+$//;
    my $val = $$cmd_ref;
    next unless $val;
    next unless $val;
    if ($val =~ /`/) {
        die "$Error Forbidden backtick for option `--$cmd' ($val)!\n";
    }
    if ($val =~ /\s/) {
        my $err = 0;
        if ($restricted or not $Win) {
            $err = 1;
        }
        else {
            $err = 1 if $val =~ /\.exe.*\s/i;
            $err = 1 if $val =~ /\s[-\/@+]/;
        }
        die "$Error Forbidden whitespace for option `--$cmd' ($val)!\n" if $err;
    }
}
if ($restricted) {
    if ($::opt_pdftexcmd and $::opt_pdftexcmd ne 'pdftex') {
        die "$Error pdfTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_xetexcmd and $::opt_xetexcmd ne 'xetex') {
        die "$Error XeTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_luatexcmd and $::opt_luatexcmd ne 'luatex') {
        die "$Error LuaTeX program name must not be changed in restricted mode!\n";
    }
    if ($::opt_gscmd) {
        $::opt_gscmd =~ /^(gs|mgs|gswin32c|gs386|gsos2)$/
        or $::opt_gscmd =~ /^gs[\-_]?(\d|\d[\.-_]?\d\d)c?$/
        or die "$Error: Invalid Ghostscript program name in restricted mode!\n";
    }
}
if ($Win and $::opt_gscmd =~ /\s/) {
    $::opt_gscmd = "\"$::opt_gscmd\"";
}

### cleanup system
my @unlink_files = ();
my $exit_code = 1;
sub clean {
    print "* Cleanup\n" if $::opt_debug;
    if ($::opt_debug) {
        print "* Temporary files: @unlink_files\n";
    }
    else {
        for (; @unlink_files>0; ) {
            unlink shift @unlink_files;
        }
    }
}
sub cleanup {
    clean();
    exit($exit_code);
}
$SIG{'INT'} = \&cleanup;
$SIG{'__DIE__'} = \&clean;

### Calculation of BoundingBoxes

# use safe file name for use within cmd line of gs (unknown shell: space, ...)
# and XeTeX (hash, curly braces, ...)
my $inputfilesafe = $inputfile;
if ($inputfile eq '-') {
    $inputfilesafe = "$tmp-stdin.pdf";
    print "* Temporary input file: $inputfilesafe\n" if $::opt_debug;
    push @unlink_files, $inputfilesafe;
    open(OUT, '>', $inputfilesafe)
            or die sprintf "$Error Cannot write `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    binmode(OUT);
    my $size = 0;
    my $len = 0;
    my $buf = '';
    my $buf_size = 65536;
    do {
        $len = read STDIN, $buf, $buf_size;
        if (not defined $len) {
            my $msg = exterr;
            die "$Error Reading standard input ($msg)!\n";
        }
        print OUT $buf
                or die sprintf "$Error Writing `%s` (%s)!\n",
                               $inputfilesafe, exterr;
        $size += $len;
    }
    while ($len);
    close(OUT);
    print "* File size (STDIN): $size\n" if $::opt_debug;
}
elsif (not $inputfile =~ /^[\w\d\.\-\:\/@]+$/) { # /[\s\$~'"#{}%]/
    $inputfilesafe = "$tmp-img.pdf";
    push @unlink_files, $inputfilesafe;
    my $symlink_exists = eval {
        local $SIG{'__DIE__'};
        symlink("", "");
        1;
    };
    print "* Input file name `$inputfile' contains special characters.\n"
          . "* " . ($symlink_exists ? "Link" : "Copy")
          . " input file to temporary file `$inputfilesafe'.\n"
            if $::opt_verbose;
    if ($symlink_exists) {
        symlink($inputfile, $inputfilesafe)
            or die sprintf "$Error Link from `%s' to `%s' failed (%s)!\n",
                           $inputfile, $inputfilesafe, exterr;
    }
    else {
        use File::Copy;
        copy($inputfile, $inputfilesafe)
                or die sprintf "$Error Copy from `%s' to `%s' failed (%s)\n",
                               $inputfile, $inputfilesafe, exterr;
    }
}

if ($::opt_pdfversion eq 'auto') {
    open(IN, '<', $inputfilesafe)
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           $inputfilesafe, exterr;
    my $buf;
    read(IN, $buf, 1024)
            or die sprintf "!!! Error: Cannot read the header of `%s' failed (%s)!\n",
                           $inputfilesafe, exterr;
    close(IN);
    if ($buf =~ /%PDF-1.([0-7])\s/) {
        $::opt_pdfversion = $1;
        print "* PDF header: %PDF-1.$::opt_pdfversion\n" if $::opt_verbose;
        $::opt_pdfversion = 2 if $::opt_pdfversion < 2;
    }
    else {
        die "!!! Error: Cannot find PDF header of `$inputfilesafe'!\n";
    }
}
print '* Using PDF minor version: ',
      ($::opt_pdfversion ? $::opt_pdfversion : "engine's default"),
      "\n" if $::opt_debug;

my @gsargs = (
    "-sDEVICE=bbox",
    "-dBATCH",
    "-dNOPAUSE"
);
push @gsargs, "-sPAPERSIZE=$::opt_papersize" if $::opt_papersize;
push @gsargs, "-r$::opt_resolution" if $::opt_resolution;
push @gsargs,
    "-c",
    "save",
    "pop",
    "-f",
    $inputfilesafe
;

my $tmpfile = "$tmp.tex";
push @unlink_files, $tmpfile;
open(TMP, ">$tmpfile")
    or die sprintf "$Error Cannot write tmp file `%s' (%s)!\n",
                   $tmpfile, exterr;
print TMP <<'END_TMP';
\catcode37 14 % percent
\catcode33 12 % exclam
\catcode34 12 % quote
\catcode35  6 % hash
\catcode39 12 % apostrophe
\catcode40 12 % left parenthesis
\catcode41 12 % right parenthesis
\catcode45 12 % minus
\catcode46 12 % period
\catcode60 12 % less
\catcode61 12 % equals
\catcode62 12 % greater
\catcode64 12 % at
\catcode91 12 % left square
\catcode93 12 % right square
\catcode96 12 % back tick
\catcode123 1 % left curly brace
\catcode125 2 % right curly brace
\catcode126 12 % tilde
\catcode`\#=6 %
\escapechar=92 %
\def\IfUndefined#1#2#3{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    #2%
  \else
    #3%
  \fi
}
END_TMP
my $pdffilehex = unpack 'H*', $inputfilesafe;
$pdffilehex = "\U$pdffilehex\E";
print TMP "\\def\\pdffilehex{$pdffilehex}\n";
print TMP <<'END_TMP';
\IfUndefined{pdfunescapehex}{%
  \begingroup
    \gdef\pdffile{}%
    \def\do#1#2{%
      \ifx\relax#2\relax
        \ifx\relax#1\relax
        \else
          \errmessage{Invalid hex string, should not happen!}%
        \fi
      \else
        \lccode`0="#1#2\relax
        \lowercase{%
          \xdef\pdffile{\pdffile0}%
        }%
        \expandafter\do
      \fi
    }%
    \expandafter\do\pdffilehex\relax\relax
  \endgroup
}{%
  \edef\pdffile{\pdfunescapehex{\pdffilehex}}%
}
\immediate\write-1{Input file: \pdffile}
END_TMP
if ($::opt_tex eq 'luatex') {
    print TMP <<'END_TMP';
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
  \errmessage{LuaTeX not found!}%
\else
  \begingroup
    \newlinechar=10 %
    \endlinechar=\newlinechar %
    \ifnum0%
        \directlua{%
          if tex.enableprimitives then
            tex.enableprimitives('TEST', {
              'luatexversion',
              'pdfoutput',
              'pdfcompresslevel',
              'pdfhorigin',
              'pdfvorigin',
              'pdfpagewidth',
              'pdfpageheight',
              'pdfmapfile',
              'pdfximage',
              'pdflastximage',
              'pdfrefximage',
              'pdfminorversion',
              'pdfobjcompresslevel',
            })
            tex.print('1')
          end
        }%
        \ifx\TESTluatexversion\UnDeFiNeD\else 1\fi %
        =11 %
      \global\let\luatexversion\luatexversion %
      \global\let\pdfoutput\TESTpdfoutput %
      \global\let\pdfcompresslevel\TESTpdfcompresslevel %
      \global\let\pdfhorigin\TESTpdfhorigin %
      \global\let\pdfvorigin\TESTpdfvorigin %
      \global\let\pdfpagewidth\TESTpdfpagewidth %
      \global\let\pdfpageheight\TESTpdfpageheight %
      \global\let\pdfmapfile\TESTpdfmapfile %
      \global\let\pdfximage\TESTpdfximage %
      \global\let\pdflastximage\TESTpdflastximage %
      \global\let\pdfrefximage\TESTpdfrefximage %
      \global\let\pdfminorversion\TESTpdfminorversion %
      \global\let\pdfobjcompresslevel\TESTpdfobjcompresslevel %
    \else %
      \errmessage{%
        Missing \string\luatexversion %
      }%
    \fi %
  \endgroup %
\fi
END_TMP
}
if ($::opt_tex eq 'pdftex' or $::opt_tex eq 'luatex') {
    print TMP <<'END_TMP_HEAD';
\pdfoutput=1 %
\pdfcompresslevel=9 %
\csname pdfmapfile\endcsname{}
\def\setpdfversion#1{%
  \IfUndefined{pdfobjcompresslevel}{%
  }{%
    \ifnum#1<5 %
      \pdfobjcompresslevel=0 %
    \else
      \pdfobjcompresslevel=2 %
    \fi
  }%
  \IfUndefined{pdfminorversion}{%
    \IfUndefined{pdfoptionpdfminorversion}{%
    }{%
      \pdfoptionpdfminorversion=#1\relax
    }%
  }{%
    \pdfminorversion=#1\relax
  }%
}
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \pdfximage page #1 mediabox{\pdffile}%
    \pdfrefximage\pdflastximage
  }%
  \pdfhorigin=-#2bp\relax
  \pdfvorigin=#3bp\relax
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \ht0=\pdfpageheight
  \shipout\box0\relax
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \count0=#1\relax
  \dimen0=#4bp\relax \advance\dimen0 by -#2bp\relax
  \edef\imagewidth{\the\dimen0}%
  \dimen0=#5bp\relax \advance\dimen0 by -#3bp\relax
  \edef\imageheight{\the\dimen0}%
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{%
    \kern -#2bp\relax
    \lower #3bp\hbox{\pdfrefximage\pdflastximage}%
  }%
  \wd0=\imagewidth\relax
  \ht0=\imageheight\relax
  \dp0=0pt\relax
  \pdfhorigin=#6pt\relax
  \pdfvorigin=#7bp\relax
  \pdfpagewidth=\imagewidth
  \advance\pdfpagewidth by #6bp\relax
  \advance\pdfpagewidth by #8bp\relax
  \pdfpageheight=\imageheight\relax
  \advance\pdfpageheight by #7bp\relax
  \advance\pdfpageheight by #9bp\relax
  \pdfxform0\relax
  \shipout\hbox{\pdfrefxform\pdflastxform}%
}%
\def\pageinclude#1{%
  \pdfhorigin=0pt\relax
  \pdfvorigin=0pt\relax
  \pdfximage page #1 mediabox{\pdffile}%
  \setbox0=\hbox{\pdfrefximage\pdflastximage}%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \raise\dp0\box0\relax
  }%
}
END_TMP_HEAD
    print TMP "\\setpdfversion{$::opt_pdfversion}\n" if $::opt_pdfversion;
}
else { # XeTeX
    print TMP <<'END_TMP_HEAD';
\expandafter\ifx\csname XeTeXpdffile\endcsname\relax
  \errmessage{XeTeX not found or too old!}%
\fi
\def\page #1 [#2 #3 #4 #5]{%
  \count0=#1\relax
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=#4bp\relax
  \advance\pdfpagewidth by -#2bp\relax
  \pdfpageheight=#5bp\relax
  \advance\pdfpageheight by -#3bp\relax
  \shipout\hbox{%
    \kern-1in%
    \kern-#2bp%
    \vbox{%
      \kern-1in%
      \kern#3bp%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
\def\pageclip #1 [#2 #3 #4 #5][#6 #7 #8 #9]{%
  \page {#1} [#2 #3 #4 #5]%
}
\def\pageinclude#1{%
  \setbox0=\hbox{%
    \XeTeXpdffile "\pdffile" page #1 media\relax
  }%
  \pdfpagewidth=\wd0\relax
  \pdfpageheight=\ht0\relax
  \advance\pdfpageheight by \dp0\relax
  \shipout\hbox{%
    \kern-1in%
    \vbox{%
      \kern-1in%
      \ht0=\pdfpageheight
      \box0 %
    }%
  }%
}
END_TMP_HEAD
}

print "* Running ghostscript for BoundingBox calculation ...\n"
    if $::opt_verbose;
print "* Ghostscript call: $::opt_gscmd @gsargs\n" if $::opt_debug;

my @bbox;
my @bbox_all;
my @bbox_odd;
my @bbox_even;
if ($::opt_bbox) {
     $::opt_bbox =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_all = ($1, $2, $3, $4);
}
if ($::opt_bbox_odd) {
     $::opt_bbox_odd =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_odd = ($1, $2, $3, $4);
}
if ($::opt_bbox_even) {
     $::opt_bbox_even =~ /([-\d\.]+) ([-\d\.]+) ([-\d\.]+) ([-\d\.]+)/;
     @bbox_even = ($1, $2, $3, $4);
}

sub getbbox ($$$$$) {
    my $page = shift;
    my $a = shift;
    my $b = shift;
    my $c = shift;
    my $d = shift;
    if ($page % 2 == 1) {
        if ($::opt_bbox_odd) {
            return @bbox_odd;
        }
    }
    else {
        if ($::opt_bbox_even) {
            return @bbox_even;
        }
    }
    if ($::opt_bbox) {
        return @bbox_all;
    }
    return ($a, $b, $c, $d);
}
my $page = 0;
my $gs_pipe = "$::opt_gscmd -dSAFER @gsargs 2>&1";
$gs_pipe .= " 1>$null" unless $::opt_verbose;
$gs_pipe .= " |";

open(GS, $gs_pipe)
        or die sprintf "$Error Cannot call ghostscript `%s' (%s)!\n",
                       $::opt_gscmd, exterr;
my $bb = ($::opt_hires) ? "%%HiResBoundingBox" : "%%BoundingBox";
my $previous_line = 'Previous line';
# Ghostscript workaround for buggy ports that prints
# the bounding box data twice on STDERR.
while (<GS>) {
    print $_ if $::opt_verbose;
    if (/^$bb:\s*(-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+) (-?[\.\d]+)/o) {
    }
    else {
        $previous_line = $_;
        next;
    }
    next if $previous_line eq $_;
    $previous_line = $_;
    $page++;
    @bbox = getbbox($page, $1, $2, $3, $4);

    my $empty = 0;
    $empty = 1 if $bbox[0] >= $bbox[2];
    $empty = 1 if $bbox[1] >= $bbox[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: Empty Bounding Box is returned by Ghostscript!
!!!   Page $page: @bbox
!!! Either there is a problem with the page or with Ghostscript.
!!! Recovery is tried by embedding the page in its original size.

END_WARNING
        print TMP "\\pageinclude{$page}\n";
        next;
    }

    print "* Page $page: @bbox\n" if $::opt_verbose;

    my @bb = ($bbox[0] - $llx, $bbox[1] - $ury,
             $bbox[2] + $urx, $bbox[3] + $lly);

    $empty = 0;
    $empty = 1 if $bb[0] >= $bb[2];
    $empty = 1 if $bb[1] >= $bb[3];
    if ($empty) {
        print <<"END_WARNING";

!!! Warning: The final Bounding Box is empty!
!!!   Page: $page: @bb
!!! Probably caused by too large negative margin values.
!!! Recovery by ignoring margin values.

END_WARNING
        print TMP "\\page $page [@bbox]\n";
        # clipping shouldn't make a difference
        next;
    }
    if ($::opt_clip) {
        print TMP "\\pageclip $page [@bbox][$llx $lly $urx $ury]\n";
    }
    else {
        print TMP "\\page $page [@bb]\n";
    }
}
close(GS);

if ($? == -1) {
    die sprintf "$Error Ghostscript failed to execute (%s)!\n",
                exterr;
}
elsif ($? & 127) {
    die sprintf  "$Error Ghostscript died with signal %d!\n",
                 ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error Ghostscript exited with error code %d!\n",
                $? >> 8;
}

print TMP "\\csname \@\@end\\endcsname\n\\end\n";
close(TMP);

if ($page == 0) {
    die "$Error Ghostscript does not report bounding boxes!\n";
}

### Run pdfTeX/XeTeX

push @unlink_files, "$tmp.log";
my $cmd;
my $texname;
if ($::opt_tex eq 'pdftex') {
    $cmd = $::opt_pdftexcmd;
    $texname = 'pdfTeX';
}
elsif ($::opt_tex eq 'luatex') {
    $cmd = $::opt_luatexcmd;
    $texname = 'LuaTeX';
}
else {
    $cmd = $::opt_xetexcmd;
    $texname = 'XeTeX';
}
$cmd = "\"$cmd\"" if $Win and $cmd =~ /\s/;
$cmd .= ' -no-shell-escape';
if ($::opt_initex) {
    $cmd .= ' --ini --etex';
}
if ($::opt_verbose) {
    $cmd .= " -interaction=nonstopmode $tmp";
}
else {
    $cmd .= " -interaction=batchmode $tmp";
}
print "* Running $texname ...\n" if $::opt_verbose;
print "* $texname call: $cmd\n" if $::opt_debug;
if ($::opt_verbose) {
    system($cmd);
}
else {
    `$cmd`;
}
if ($? == -1) {
    die sprintf "$Error %s run failed to execute (%s)!\n",
                $texname, exterr;
}
elsif ($? & 127) {
    die sprintf "$Error %s run died with signal %d!\n",
                $texname, ($? & 127);
}
elsif ($? != 0) {
    die sprintf "$Error %s run failed with value %d!\n",
                $texname, ($? >> 8);
}

### Check pdf version of temp file
if ($::opt_pdfversion) {
    open(PDF, '+<', "$tmp.pdf")
            or die sprintf "!!! Error: Cannot open `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    my $header;
    read PDF, $header, 9
            or die sprintf "!!! Error: Cannot read header of `%s' (%s)!\n",
                           "$tmp.pdf", exterr;
    $header =~ /^%PDF-1\.(\d)\s$/ or die "!!! Error: Cannot find header of `$tmp.pdf'!\n";
    if ($1 ne $::opt_pdfversion) {
        seek PDF, 7, 0
                or die sprintf "!!! Error: Cannot seek in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print PDF $::opt_pdfversion
                or die sprintf "!!! Error: Cannot write in `%s' (%s)!\n",
                               "$tmp.pdf", exterr;
        print "* PDF version correction in output file: 1.$::opt_pdfversion\n"
                if $::opt_debug;
    }
    close(PDF);
}

### Move temp file to output
if (!rename("$tmp.pdf", $outputfile)) {
    use File::Copy;
    move "$tmp.pdf", $outputfile or
            die "$Error Cannot move `$tmp.pdf' to `$outputfile'!\n";
}

print "==> $page page", (($page == 1) ? "" : "s"),
      " written on `$outputfile'.\n";

$exit_code = 0;
cleanup();

__END__


==> misc/design-counting-old.tex <==
% !TeX root = main.tex
\subsection{Executing counting queries}
Counting queries aims to get the statistics of a certain object class through a long period of time, e.g., max, average, and median.

\paragraph{Overall Workflow of Max Counting}
\note{already covered}
Instead of using multi-class classification to count the number of object in a specific frame, \sys{} is consistent with rankers used in the retrieval queries that returns a higher confidence when there are more objects in the frame.
The camera prioritizes the frames with higher chances of having more objects to upload until the user terminates the query.
\note{does this challenge our design? why do we care about this}
One key difference between max counting query and retrieval query is that the max frame may appear only once in the whole time range.


\noindent $\bullet$ \textit{Bootstrap}
\note{what's unique here? seems same as other cases}
After user issues the query, the cloud will first retrieve the low-resolution landmark frames and their tagged results from the camera.
A set of specialized operators will be trained by turn from cheap to expensives.
The label of a specific training frame is a floating number between [0,1], and the larger the value, the higher confidence that the frame will contain more objects.
The metric of choosing the first operator is quite similar to retrieval.

\noindent $\bullet$ \textit{Rank}
After shipping the first operator to the camera, and starts processing frames randomly.
The processed frames is ranked by their scores from high to low be in a priority queue.
At the meantime, \sys{} keeps uploading the top frame.
After finish ranking all the frames, the operator will be replaced by a more accurate but slower operator.

\note{how to choose init op?}

\noindent $\bullet$ \textit{Upgrade}
While the camera is busy ranking the frames, the cloud keeps training more expensive operators that is ready for future upgrades.
Similar to retrieval, \sys{} then selects the most accurate one which runs no $\eta \times$ slower than the net/opspeed ratio of the previous operator.
\note{when to upgrade?}

\noindent $\bullet$ \textit{Re-rank and loop-back}
After shipping the new operator to the camera, \sys{} starts to process the remaining frames based on the ranked result in the legacy priority queue by the predecessor operator.
The ranking result will be stored in new priority queue, and the top frame is kept uploading to the cloud.
\note{same as generic}

%\begin{myitemize}
%\item avg/sum random sampling with filtering (?)
%\item percentile: random sampling with filtering? 
%\item max: 
%max seems a bit special. It is not aggregation. 
%ranking. discover the most likely frames that contain max
%\end{myitemize}

\paragraph{Overall Workflow of Average/Median Counting}
Statistically, the average and median are always estimated through uniform sampling. \note{cite -- elaborate this clearly} 
Different from max counting that we need to rank and prioritize the frame to upload to the cloud, statistics like average and median embraces the diversity of frames instead of the skewness.
Starting from the landmark frames that are tagged at ingestion time, the camera continuously uploads the frames sampled from the queried time range until it get converged.
Our evaluation in Section \note{xxx} shows that the accuracy and sparsity of landmark frames has a large impact on the accuracy of accumulated statistics, and landmark with shorter intervals and more accurate results tends to converge earlier.

\note{clarify: at query time we do not run any on-camera op. and justify. }

\note{are we providing running error as the query execution proceeds}

==> misc/design-retrieval-old.tex <==
% !TeX root = main.tex
\subsection{Executing retrieval queries}

\note{covered. merged pos/negs to earlier}
Retrieval query is used to obtain the image frames that contain certain taget object or features. We call those frames as positive frames, and others as negative frames vice versa.

\note{there is semantics mapping. covered}
\noindent \textbf{Overall workflow}: \sys{} uses binary operators to prioritize the frames being sent from camera to cloud. The cloud will then run cloud oracle model on the sent frames and display the positive ones to users. The binary operators will score each frame, with higher scores indicating a higher chance that the frames is positive.
In essence, it's about how to prioritize the frames to be sent.

\noindent $\bullet$ \textit{Step-0:}
After user issues the query, the cloud will first retrieve the landmark frames (low-resolution) and their tagging results from camera.
A set of specialized operators will be trained based on those frames.
\sys{} will then select the initial operator based on the following policy: selecting the most accurate operator with $[op\_fps \times pos\_ratio > net\_fps]$.
The rationale is that if the binop explores $op\_fps$ frames per second, we estimate the binop will encounter $op\_fps \times pos\_ratio$ frames per second. 
We would like that number to be no less than the upload bandwidth, otherwise we will knowingly upload negative frames.
Here, $pos\_ratio$ can be estimated from landmark frames.
The metric of operator accuracy used in retrieval query is AUC.

\noindent $\bullet$ \textit{Step-1:}
The selected operator will be deployed on camera, and starts processing frames randomly.
The processed frames along with their scores will be stored in a priority queue.
Asynchronously, \sys{} keeps sending highest-score frames from the priority queue to the cloud.
This operator will be discarded and upgraded when it has finished processing every remaining frames, or the cloud tells that the recent frames being sent are in low quality, e.g., 2X lower positive ratio than the first sent ones. \note{elaborate}

\noindent $\bullet$ \textit{Step-2:}
When upgrading operators, the cloud will re-train a list of operators based on both landmark frames and the frames newly sent.
It then selects the most accurate one which runs no $\eta \times$ slower than the previous operator.
In other words, we loose the speed constrain so that a slower but more accurate operator will be deployed.
Here, $\eta$ is a decay factor which is empirically determined.

\note{Is it adaptive? -- please use net/op speed ratio}

\noindent $\bullet$ \textit{Step-3:}
The new operator will be downloaded to camera, and starts to process the remaining frames immediately.
The order of processing is based on the frame score given by previous operator, i.e., the old priority queue.
The frames processed by the current operator will be stored in a new priority queue, which will be consumed by the network bandwidth.
\note{covered}

\noindent $\bullet$ \textit{Step-4:}
Iterate the above process until the user stops the query or all the frames have been returned.

During the query process, \sys{} only considers operators runs faster than network, so that the network bandwidth is never starved.
Notice that every frame will be sent to cloud and confirmed by the cloud oracle model (which we regard as ground truth), so that there will be no error (false positive frames) returned to users.
\note{covered. perhaps worth reminding though}


%
%\noindent \textbf{Ranking task}: to minimize end-to-end latency, we keep sending frames from camera to cloud, and run the cloud oracle model to verify the sending frames (thus no error). In essence, it's about how to prioritize the frames to be sent.
%
%\noindent \textbf{Optimization goal}: how fast we can return N\% positive frames that contain the target object (frame-centric) or different instances of target object (instance-centric) to users. The number of N is not likely to be given by user in practice, thus we need to optimize the overall retrieval process, e.g., N = 50, 80, 99, etc.
%\note{what does this mean? If N is unknown, how can we opt}
%
%
%\st{Multi-stage shallow NNs}
%\paragraph{Multi-pass ranking -- non-blocking}
%We notice that there's no golden policy to select an optimal model that exhibit the best performance over the whole retrieval process. Some of them are good at quickly returning 50\% frames (fast, inaccurate NNs), some of others are good at returning 90\% (slow, accurate NNs). 
%
%each pass builds on the results of the previous pass.
%
%\note{Mengwei: elaborate why 90\% is not as good.} Too slow in confirming high-confidence frames? Does not maximize the uploading rate of positive samples. 
%\textbf{xzl: It's better to send a mixture of good/bad things from a large scope than sending only good things from a smaller scope.} 
%
%\note{How do we decide planning horizon?}
%
%Thus, we use a multi-stage retrieval procedure where multiple NNs are engaged (Figure~\ref{fig:retrieval-multi}).
%\begin{enumerate}
%
%\item Starting from the most accurate model which runs faster than a \textbf{speed limit}. We use it to quickly rank the frames \textit{randomly}.
%
%\item Cloud monitors the frames sent from camera. If too much garbage (e.g., 2X lower positive ratio than the first sent ones), we loose the speed limit, and choose a slower but more accurate model to update the ranking results. This time, we rank the frames based on the priority given by the previous NN rather than randomly. \note{An interesting observation from experiments: for instance-centric retrieval, it's better to abandom the previous prioritization but run the new NN on the remaining frames randomly.}
%\item Iterating the above process until user stops the query or all frames have been returned.
%
%\item \textbf{Op upgrade}. the second op (which still runs faster than net bw), once downloaded, starts to rank. 
%Since the second op outpaces network bw, from this moment onward the cam always upload frames ranked by the second op. 
%From this POV, upgrading to the op that has highest accuracy make sense. 
%\end{enumerate}
%
%\note{Possible that an op runs slower than bw but has good accuracy so that its upload rate of ``good'' data is actually higher?}
%
%\textbf{Adjacent positive frames identified by optical flow}. For frame-centric 
%
%\note{idea} Can temporal locality learnt from LM further help this? 
%
%\textbf{Key planning question: How do we pick on-cam ops?} 
%for retrieval, everytime we specify a speed limit, and select the most accuracte one that runs faster than this limit; 


==> misc/design-tagging-old.tex <==
% !TeX root = main.tex
\subsection{Executing tagging queries}
\note{covered}
Tagging query is used to understand the appearance duration of certain objects, e.g., when does a deer show up in the video (how many times, how long each time, etc)?

\noindent \textbf{Overall workflow}:
\note{covered}
\sys{} uses the same kind of binary operators as in retrieval. The duty of those operators, however, are different.
Instead of ranking, \sys{} uses operators as filters: the frames with high or low scores will be tagged directly, while the uncertain frames will be sent to cloud to be tagged by cloud oracle model.

\note{this is how to sample}
\sys{} treats the tagging process as a multi-stage refinement process: at each refinement level, there is at least one frame tagged every $K$ sequential frames ($K$ = 30, 10, ..., 1). We call $K$ the group size.

\noindent \textit{Step-0:}
As retrieval, \sys{} first uses landmark frames to train a list of operators (bootstrap).
\note{covered}
For each operator, two thresholds will be set to satisfy the user-defined error.
The frames with score higher than $T\_high$ will be tagged as positive directly, while the frames with score lower than $T\_low$ will be regarded as negative.
The thresholds are determined based on a testing frame set.

\note{important}
\sys{} then selects the first operator with highest $[op\_fps \times tag\_ratio + net\_fps]$, where $tag\_ratio$ is the \% of frames the op can tag, an indicator of the operator accuracy.
We call this metric as effective tagging ratio of this operator.
The rationale behind is that the selected operator has the highest tagging speed which is related both its speed and accuracy.

\noindent \textit{Step-1:}
The job of each deployed operator can be roughly divided into two parts.

Meanwhile, the frames in the uploading queue will be continuously uploaded to cloud and tagged by cloud oracle model.

\note{overview the idea}

First, it starts to scan each group ($K$ sequential frames) to tag frames. 

\note{perhaps need an algo list}
For each group:

\textbf{Scanning Algorithm-}
\begin{myitemize}
\item If there already exists a frame that has been tagged as positive ($P$) or negative ($N$), advance to the next group;
\item If there is existing frames marked as uncertain ($U$), add it to the uploading queue and move to the next group.
\item Otherwise (no frames has been processed), it picks a frame to process. If it can be tagged ($P$ or $N$), tag it. If it's uncertain, mark it ($U$), add it to uploading queue, and move to the next group.
\end{myitemize}

After the scanning, if the uploading queue is empty, we have resolved this refinement epoch. Otherwise, \sys{} will use the operator to revisit the groups that has no frame tagged or uploaded.

\textbf{Revisiting Algorithm-}
If the uploading queue is non-empty, we go back to the uploading queue and scan from the queue tail. 
\begin{myitemize}
\item For a frame F, locate its enclosing group; pick another frame F1 (which must be unresolved otherwise we are done for this group) to process. 
\item If F1 is $P$/$N$, tag it and remove F from the uploading queue;
\item If F1 is uncertain, tag it with $U$ and keep F in the uploading queue as F still needs to be resolved; 
go to the next frame in the uploading queue. 
\item Repeat until we finish scanning the upload queue.
\end{myitemize}

After this pass, we revisit the uploading queue if it is still not empty. 
\sys{} will repeat the revisiting algorithm above, which means it will look at another frame from the unresolved groups, hoping to resolve it.



\noindent \textit{Step-2:}
When one refinement epoch has been done, i.e., at least one frame in each group has been tagged as $P$ or $N$ either by on-camera operator or cloud, we reset the group size to a smaller one (e.g., 10 $\rightarrow$ 5). The list of group size is pre-defined.
The uploading queue will be cleared, but all the marks ($P$, $N$, and $U$) will be kept.
Then it repeats the above process.

\noindent \textit{Step-3:}
\note{important}
The operator will be upgraded under two circumstances. One is that the operator has processed every frame. The second is when the cloud realizes that the newly generated operators have much higher effective tagging ratio than the old one (e.g., 2X).
The new operator will be selected as the one with highest effective tagging ratio on the frames that have been recently uploaded.
Since the remaining frames tend to be more difficult to be resolved as the query goes on, the operators will be upgraded to slower but heavier ones.
When a new operator is deployed, both the uploading queue and uncertain frame marks ($U$) will be cleared, and the above algorithms will be repeated.

\noindent \textit{Step-4:}
Iterate the above process until the user stops the query or all the frames have been tagged.

%
%
%\paragraph{Formulating the query latency}
%
%\paragraph{plan}
%Every $N$ frames, the camera picks one for tag. 
%Randomly pick one until there is one above the confidence threshold. 
%
%\paragraph{scheduling for uploading}
%The idea is to opportunisitically uploading uncertain frames from \ul{this} planning horizon. 
%
%\textbf{Rationale}: spread local \& cloud computation effort evenly among all epochs. 
%Do not work on one single epoch for long.
%
%
%\textbf{Algorithm 1}
%
%Scan all epochs (groups) in sequence. 
%For each group: 
%\begin{myitemize}
%\item if there exists Y/N, advance to the next group;
%\item 
%if there is existing (?), mark it to be uploaded (add to the uploading queue); go to the next gruop; 
%\item 
%otherwise (all (X)), picks a frame to process. if (?), add to uploading queue same as above; 
%if Y/N, tag it and move to the next group; 
%\end{myitemize}
%
%Meanwhile, uploading (cloud workqueue) is ongoing...
%
%After the first pass, if the uploading queue is empty, each epoch has at least 1 frame resolved. We are done.
%
%\textbf{Algorithm 2}
%
%If the uploading queue is non-empty... Go back to the upload queue and scan from the queue tail. 
%\begin{myitemize}
%\item For a frame F, locate its enclosing group; pick another frame F1 (which must be unresolved (X) otherwise we are done for this group) to process. 
%\item if F1 is Y/N, tag it; remove F from the upload queue (we do not need to resolve F in this round (not horizon));
%\item If F1 is (?), tag it locally; keep F in the upload queue as F still needs to be resolved; 
%go to the next frame in the upload queue. 
%\item Repeat until we finish scanning the upload queue.
%\end{myitemize}
%
%After this pass, we revisit the uploading queue if it is still not empty. 
%Repeat algorithm 2 above. The result: we will look at another frame from \textbf{the unresolved epoch}, hoping to resolve it. 
%
%\textbf{By doing so}
%after multiple rounds, the ones still in the upload queue are from the epochs/groups where the local cam still cannot find resolvable images. 
% we automatically shift focus (resource/attention) to the epochs that are difficult to resolve, by trying more frames from these epochs.
%
%\paragraph{When to upgrade binop?}
%The cloud knows: 
%\begin{myitemize}
%\item 
%the (?) frames uploaded from the cam to be resolved
%\item 
%num of frames resolved locally on cam
%\item 
%num of frames attempted by cam but failed to resolve.
%\end{myitemize}
%
%\paragraph{Mechanism}
%Define a metric: 
%$F$ = effective local tagging fps + the rate of upload frames.
%\note{However, upload rate is often much lower than tagging rate}
%The rate of effective tagged frames is the ``net'' output of local binop. 
%It does not include frames attempted but remain unresolved. 
%
%The cloud monitors F. 
%Based on recently uploaded frames (unresolved by cam's binop), the cloud picks the binop that yields highest F. 
%
%\begin{myitemize}
%\item 
%Initially, the binop runs fast and quickly tags (easy) frames at high rate; it also discovers unresolved frames at high rate and saturates the uplink. F is high. 
%
%\item 
%As query proceeds, the binop finds increasingly difficult to tag frames locally; uplink is saturated. F drops. 
%The cloud sends a slower op, which has high confidence to tag more frames locally. F comes back. 
%
%\item 
%If network bandwidth goes high? 
%Suddenly the local bin op may not be able to saturate bw. 
%The cloud ships an op that runs faster (potentially higher rate of which exploits the ample bw to achieve higher F.  
%
%\end{myitemize}
%
%the cloud monitors the metric. if the metric starts to decline, ship a new op. 
%
%\paragraph{How to pick the new op?}
%The cloud runs all ops on recently uploaded frames. 
%These are unresolved by cam binop. 
%For each candidate binop, the cloud estimates its F 
%(If candidate op is larger than current op --
%current op: S fps; where p is resolved and S-p unresolved. 
%candidate op: S1 fps; where p + p1 resolved and S-p-p1 unresolved.)
%What if candidate op is smaller than current op?
%
%The cloud picks the op with the highest F. 
%
%It tests all binops on the unresolved frames uploaded.
%If we assume the uplink is always the bottleneck (much slower than local binop)
%It finds out the binop in the portfolio that leads to the greatest reduction in upload time, but the oncam speed is not too slow to starve the upload queue. 
%The it picks the binop for upgrade. 
%\note{the rough idea. need to refine.}

==> misc/fig-sample-minipage.tex <==
% !TeX root = main.tex

\begin{figure}[!t]

	\begin{minipage}[b]{0.23\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/fair/cpu/cpu}
		        \subcaption{CPU}
		\label{fig:gull}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/dsp/dsp}
		        \subcaption{DSP}
		\label{fig:tiger}
	\end{minipage}	

	\begin{minipage}[b]{0.23\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/fair/gpu/gpu}
		        \subcaption{GPU}
		\label{fig:tiger}
	\end{minipage}	
	~
	\begin{minipage}[b]{0.23\textwidth}
	%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
	\includegraphics[width=1\textwidth]{figs/plot/fair/wifi/wifi}
	        \subcaption{WiFi}
	\label{fig:tiger}
	\end{minipage}	
		
	\caption{Throughputs of co-running app instances, before and after one instance (marked with *) enters \psbox{}. 
%	\psbox{} ensures fairness by keeping throughputs of other apps largely unchanged.
	}
%	\vspace{-10pt}		% use as needed
	\label{fig:fair}
\end{figure}

==> misc/fig-sample-multi.tex <==
% !TeX root = main.tex

\begin{figure*}

	\captionsetup[subfigure]{labelformat=empty,justification=centering} % xzl
	
	\quad \quad \quad
	\begin{minipage}[b]{0.9\textwidth}
		\includegraphics[width=1\textwidth]{figs/power-top}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%	\centering					
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{CPU}}
		\end{picture}
	\end{minipage}	
	~			
	\centering				
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib_alone.pdf}
		\subcaption{\textbf{calib3d} \\ 936mJ}
%		\label{fig:tiger}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calibX+body.pdf}
		\subcaption{\textbf{calib3d} [w/ body] \\ 922mJ (-1.5\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calibX+dedup.pdf}
		\subcaption{\textbf{calib3d} [w/ dedup] \\ 925mJ (-1.2\%)}
%		\label{fig:mouse}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib+body.pdf}
		\subcaption{\textbf{calib3d} [w/ body] \\ 853mJ (-8.9\%)}
%		\label{fig:mouse}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/cpu/calib+dedup.pdf}
		\subcaption{\textbf{calib3d} [w/ dedup] \\ 804mJ (-14.1\%)}
%		\label{fig:mouse}
	\end{minipage}    	
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{DSP}}
		\end{picture}
	\end{minipage}	
	~		
    \centering
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm_alone.pdf}
%        \caption{wingrep \makalu{}}
		\subcaption{\textbf{dgemm} \\ 3018mJ }
        \label{fig:gull}
    \end{minipage}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{minipage}[b]{0.18\textwidth}
%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemmX+sgemm.pdf}
		\subcaption{\textbf{dgemm} [w/ sgemm] \\ 2906mJ (-3.7\%)}
        \label{fig:tiger}
    \end{minipage}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemmX+monte+sgemm.pdf}
		\subcaption{\textbf{dgemm}[w/monte+sgemm] \\ 2959mJ (-2.0\%)}
%        \label{fig:mouse}
    \end{minipage}
    ~
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm+sgemm.pdf}
		\subcaption{\textbf{dgemm} [w/ sgemm] \\ 1560mJ (-48.3\%)}
%        \label{fig:mouse}
    \end{minipage}    
	~
    \begin{minipage}[b]{0.18\textwidth}
        \includegraphics[width=1\textwidth]{figs/plot/power/dsp/dgemm+monte+sgemm.pdf}
		\subcaption{\textbf{dgemm}[w/monte+sgemm] \\ 1110mJ (-63.2\%)}
        \label{fig:mouse}
    \end{minipage}    
%    \vspace{-10pt}		% use as needed
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{GPU}}
		\end{picture}
	\end{minipage}	
	~	
	\centering
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser_alone.pdf}
		\subcaption{\textbf{browser} \\ 201mJ}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		%		\includegraphics[width=\textwidth]{figs/plot/scalability/wingrep.pdf}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browserX+magic.pdf}
		\subcaption{\textbf{browser} [w/ magic] \\ 199mJ (-0.9\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browserX+tri.pdf}
		\subcaption{\textbf{browser} [w/ triangle] \\ 201mJ (0\%)}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser+magic.pdf}
		\subcaption{\textbf{browser} [w/ magic] \\ 211mJ (+5.0\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/pvr/browser+tri.pdf}
		\subcaption{\textbf{browser} [w/ triangle] \\ 172mJ (-14.4\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.03\textwidth}	
		\begin{picture}(0.01,10)
		  \put(0.01,50){\rotatebox{90}{WiFi}}
		\end{picture}
	\end{minipage}	
	~	
	\centering
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links_alone.pdf}
		\subcaption{\textbf{browser} \\ 267mJ}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/linksX+scp.pdf}
		\subcaption{\textbf{browser} [w/ scp]\\ 273mJ (+2.2\%)}
	\end{minipage}
	~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
	%(or a blank line to force the subfigure onto a new line)
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/linksX+wget.pdf}
		\subcaption{\textbf{browser} [w/ wget] \\ 313mJ (+17.2\%)}
	\end{minipage}
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links+scp.pdf}
		\subcaption{\textbf{browser} [w/ scp] \\ 412mJ (+35.2\%)}
	\end{minipage}    
	~
	\begin{minipage}[b]{0.18\textwidth}
		\includegraphics[width=1\textwidth]{figs/plot/power/wifi/links+wget.pdf}
		\subcaption{\textbf{browser} [w/ wget] \\ 455mJ (+41.3\%)}
	\end{minipage}    
	
	\caption{\textbf{Power of the benchmark scenarios}. In all plots, x-axis: Time/Sec; y-axis: Power/Watt.
%		Each row shows a set of scenarios that test a particular driver.
%		Each row corresponds to the results of a particular driver.
%		Column 1: one app runs alone; 
%		Column 2 -- 5: the app co-runs with other apps. 
		In each row: even as an app co-runs with different apps (column 2--5), \psbox{} provides it with consistent power observations (column 2 \& 3), which are close to the power of the app running alone (column 1).
		This contrasts to the power attributed to the app by an existing accounting approach (column 4 \& 5).
		The numbers under each plot show the app's total energy and the difference compared to the energy when the app runs alone.
		Some plots cannot display full length of power activities due to space limit.
		}
	\label{fig:power}
	\vspace{-10pt}
\end{figure*}


==> misc/fig-sample-single.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
%\includegraphics[width=0.45\textwidth{}]{./figs/benchmarks} 
\missingfigure[figwidth=6cm]{Kernel support}
\vspace{-10pt}		% use as needed
\caption{This is the caption figure}
\label{tab:benchmarks}
\vspace{-20pt}		% use as needed
\end{figure}


==> misc/fig-sample-subfigure.tex <==
% !TeX root = main.tex

\begin{figure}[t!]
\centering
   \begin{subfigure}[b]{0.4\textwidth}
   \includegraphics[width=1\linewidth]{figs/plot/motiv/spatial/both4/power}
   \caption{Total CPU power of two co-running process instances, one on each core, compared to 2$\times$ power of one instance running alone. Hardware: 2$\times$core Cortex-A15}
   % Benchmark: cpp drawing tutorial 1
	\vspace{2mm}
   \label{fig:motiv:spatial} 
	\end{subfigure}
% /home/xzl/Dropbox/private/drafts/powersandbox/results/motiv/async/pvr/waterfall_without/plot
	\begin{subfigure}[b]{0.4\textwidth}
	   \includegraphics[width=1\linewidth]{figs/plot/motiv/async/pvr/waterfall}
	   \caption{A sequence of three GPU commands (top) and the total GPU power (bottom).
	   Commands of the same type have the same color. Hardware: PowerVR SGX544MP}
		\vspace{2mm}
	\end{subfigure}
	\begin{subfigure}[b]{0.4\textwidth}
	   \includegraphics[width=1\linewidth]{figs/plot/motiv/dvfs/power}
	   \caption{Comparison of CPU power of the same app when it runs after a CPU idle period and when it runs after a busy period. 
%	   CPU same as (a)
	   }
	\end{subfigure}

\caption{\textbf{Examples of power entanglement}}

\vspace{-10pt}		% use as needed

\label{fig:motiv}
\end{figure}

==> overview-mwx.tex <==
% !TeX root = main.tex

%\section{An Overview of \sys{}}
\section{The \sys{} Overview - mwx}
%\section{A case for \sys{}}
%\section{The \sys{} Design}
\label{sec:overview-mwx}

\paragraph{Query types}
\sys{} targets ad-hoc video queries extensively studied in prior work~\cite{focus,noscope,blazeit,vigil}. 
%Table~\ref{tab:query} summarizes the query types. 
Concerning a specific camera, 
a query ($\mathcal{T, C}$) covers a video timespan $\mathcal{T}$, typically hours or days, and 
an object class $\mathcal{C}$ as recognizable by modern NNs, e.g., any of the 80 classes of YOLOv3~\cite{yolov3}.
The query parameters cannot be enumerated ahead of query time. 
As summarized in Table~\ref{tab:query}, 
\sys{} supports three query types 
\textbf{\textit{Retrieval}}, 
e.g., ``retrieve all images that contain yellow buses from yesterday'';
\textbf{\textit{Tagging}}, 
e.g., ``return all time ranges when any deer shows up in the past week'', 
for which the time ranges are represented as metadata but not images;
\textbf{\textit{Counting}},
e.g., ``return the maximum number of cars that ever appear in any frame today''.


\sys{} runs on both a low-cost camera and a cloud.
A limited network bandwidth is only provisioned at query time.
Regarding the query latency, the limited computing power of camera and the network bandwidth constitute the bottleneck instead of the computing power of cloud which can be easily scaled up.
\sys{} is built atop three key ideas.

\Note{Overview is not the place for key ideas, which shall be covered in intro already}

\paragraph{First key idea ($\S$\ref{sec:lm}): landmarks}
at capture time, \sys{} builds \textit{rough knowledge} of the video by running accurate object detector on sparse frames, e.g., one in tens of seconds.
We call those frames as \textit{landmarks}.
The knowledge is mainly twofolded.
\textbf{\textit{(i): spatial distribution}}: e.g., 
``90\% of the buses appear in a 200x200 region''.
\textbf{\textit{(ii): temporal distribution}}: e.g., 
``most of the people appear during daytime''.
Later in the query time, such knowledge serves as a key optimization to speedup query execution.
Furthermore, the landmarks with their object labels are used as initial training samples for bootstrapping specialized NNs \Note{what's special NN? not introduced} on-the-fly.
For Counting query, the landmarks also provide initial estimation of statistics by counting the object labels on the collected landmarks. 
\Note{unclear who is using landmarks, camera or cloud?}

\paragraph{Second key idea ($\S$\ref{sec:op}): operator upgrade}
At query time, \sys{} runs specialized NNs (called operators) on cameras to identify the target object \Note{sounds like we are detecting objects but we are not}.
Specializing NN for video and object type is a well-known technique~\cite{noscope,blazeit}.
However, we are the first to observe the opportunity of running multiple operators iteratively on the same set of video frames.
The rationale is that different frames have different difficulty to be accurately processed, and different operators exhibit rich accuracy-speed trade-offs.
Thus, instead of selecting on single operator as prior work does, \sys{} runs cheap operator to resolve the easy frames first, and then selectively upgrades the operator to resolve the rest of frames, until query finishes.
In such a way, the average \textit{cost} of resolving each frame is reduced and the overall query latency is highly optimized.
%\sys{} further enhances the operators by exploiting the spatial skewness learned from landmarks.

To fit the semantics of different query types, operators act as different roles.
%\textit{Retrieval} and \textit{\countmax} $\rightarrow$ \textit{rankers} on camera. 
%\textit{Rankers} (Figure~\ref{fig:exec} (a)): 
%for \textit{Retrieval} and \textit{\countmax} queries.
%As shown in Figure~\ref{fig:exec} (a),
(1) For \textit{Retrieval} queries and \textit{\countmax} queries, operators are \textit{rankers}.
A ranker scores frames; 
a higher score suggests that the frame is more likely to contain \textit{any} object of the queried class (for Retrieval) or \textit{a large count} of such objects (for \countmax{}).
The camera uploads ranked frames in descending order. 
(2) For \textit{Tagging} queries, operators are \textit{filters}.
A filter is trained with a pair of numerical thresholds;
the filter resolves any frame scored below/above the thresholds as negative/positive; 
the filter deems other frames as unresolved. 
Accordingly, 
the camera uploads a one-bit positive/negative tag for each resolved frame; 
the camera either uploads unresolved frames for the cloud to decide or defer them to more accurate filters on camera. 

\Note{this is about query semantics and shall be discussed prior to landmarks etc}

\paragraph{Third key idea ($\S$\ref{sec:design}): delivering results while executing}
With weak cameras and large videos, executing a query to the full is likely to take long. 
%We therefore retrofit the idea of online query processing~\cite{control}: while executing a query, 
\sys{} adopts online query processing~\cite{control}, by 
emitting partial results (e.g. approximate object counts) early, continuously refining the results, 
and reporting query progress.
Accordingly, 
the query performance is characterized as the rate of query result converging to the exact answer.
Table~\ref{tab:query} summarizes the user's view of query results and performance metrics.
Online processing suits video exploration targeted by \sys{}: 
it amortizes a query's high delay over many installments of results;
it pipelines query execution with user thinking~\cite{eureka};
%seeing early results, 
it enables a user to interactively explore a video, e.g., by aborting a query, revising parameters, and issuing anew~\cite{ola,eureka}.
While online query processing has been used for taming large datasets~\cite{olamr,online-mapreduce},
% \st{(e.g. relational databases \note{cite} and map reduce \note{cite})} 
we are the first applying it to visual data to our knowledge.  


\paragraph{Execution workflow}
Figure~\ref{fig:design-execution} shows a generic workflow of query execution.
Upon receiving a query, the cloud retrieves all landmarks in the queried video range. 
The camera ships landmarks as low-resolution thumbnails (e.g., 100$\times$100) annotated with object labels and bounding boxes
(\circled{1}).
Using the landmarks, the cloud bootstraps a family of operators (\circled{2}) and picks the initial one for the camera.
The camera executes the operators to filter or rank queried frames and uploads the ranked or surviving frames (\circled{3}). 
On the uploaded frames, 
the cloud runs generic, high-accuracy object detection and  materializes query results (e.g. positives image frames).
It also uses the processed frames to further train the candidate operators for higher accuracy (\circled{4}).
Based on the observed quality of uploaded frames, the cloud triggers upgrading of on-camera operators (\circled{5}).  
With the new operator, the camera continues to process the remaining frames (\circled{6}).
Step (\circled{4})--(\circled{6}) repeat until query abort or completion. 
Throughout the query, the cloud keeps presenting the refined result to the user (\circled{7}).

% There are multiple notable designs. 
% (1) 
% The cloud trains same-type operators with diverse costs and accuracies;
% %e.g. slower rankers that rarely gives low scores to true positive frames 
% %and a fast ranker that will mistakenly score many true positives low. 
% (2) 
% The cloud keeps training operators throughout a query's execution rather than in one shot. 
% (3)
% The camera processes frames in multiple passes, one operator in each pass. 
% (4) 
% %the camera executes its compute and frame upload in parallel.
% The camera processes and uploads the same set of frames asynchronously.
% %This is because uploading cannot wait for sort to complete, which may takes as long as hours.
% %This is because our goal of progressive execution: user demands to see results as the camera processes.
% For instance, 
% when the camera finishes ranking 100 out of total 1000 frames, it may have uploaded the top 50 of the 100 ranked frames. 
% %Hence, the rankers are \textit{non-blocking} as 
% This is opposed to common ranking that would hold off frame upload until all the frames are ranked~\cite{rank-aware-opt,similarity-join,koudas2000high}. 
% It hence ensures online processing.

==> recycle/recycle-bkgnd.tex <==
% !TeX root = main.tex

%\section{Background \& Motivations}
\section{Motivations}
\label{sec:bkgnd}

%\subsection{A case for retro analytics over on-camera videos (``reactive''/quiet cameras)}



\subsection{The camera hardware}

%We are witnessing the prosperity of low-cost cameras
%typically under \$40 per unit. 

%For example, WyzeCam (\$20) is reported to ship a quarter-million units in less than six months~\cite{wyzecam-success}. 
%Some of them can execute lightweight analytics, e.g. pedestrian detection~\cite{wyze-camv2}. 
%On-camera analytics start to emerge as key features, 
%e.g. pedestrian detection on WyzeCam~\cite{wyze-camv2}. 
%We make two observations of their hardware specs. 

\paragraph{Compute resource is frugal}
Low-cost cameras (<\$40) are typically equipped with embedded CPU cores, e.g., Cortex-A9 for YI Home Camera~\cite{yi-cam} and Ingenic T20 (MIPS32) for WyzeCam~\cite{wyze-camv2}; 
their DRAM is no more than a few GBs~\cite{wyzecam, cheapcam}. 
They are only capable of lightweight video processing~\cite{wyze-camv2}.
%Only lightweight analytics is possible on camera~\cite{wyze-camv2}.
%Some of them can execute lightweight analytics, e.g. pedestrian detection~\cite{wyze-camv2}. 
% YI home cam: Ambarella S2LM
%

% Cheap NN accelerators, e.g., HiSilicon NPU~\cite{hisilicon-npu} \Note{remove this citation}, are emerging but yet to be integrated into the majority of cameras. 

\input{tab-storage}

\paragraph{Storage is increasingly ample}
Even at low prices, 
these cameras can store large videos thanks to denser and cheaper flash storage. 
\Note{Mengwei: update the following sentence with 2020 data. Okay to use 256GB}
From 2017 to 2019, the price of MicroSD cards drops by more than 2$\times$, e.g., to \$10 (64GB) and \$23 (128GB) per card~\cite{camel-sdcard-64GB,camel-sdcard-128GB}.
%720p at 30FPS -- ~5GB per day
%Such a card holds several weeks of video footage (720p at 30 FPS, a typical format preferred by human analysts)~\cite{fortinet-white-paper}. 
Such a card holds video footage for weeks or months;
the video may be in human preferred quality, e.g. 720p at 30 FPS~\cite{fortinet-white-paper} or algorithm preferred quality, e.g. 720p at 1 FPS~\cite{focus,noscope}. 
Such video lifespans are adequate for extensive retrospective query scenarios \Note{cite?}; 
the lifespans will continue to grow as embedded flash becomes cheaper.
\Note{Please check all the numbers and citations}


%a 64GB (128GB) MicroSD card dropped from \$23 (\$45) to \$10 (\$18)~\cite{camel-sdcard-64GB,camel-sdcard-128GB}. 
%A 128GB card is capable of holding more than one month of video footage (720p at 1 FPS)~\cite{fortinet-white-paper}. % ~5GB per day
%Such a card is capable of holding $\sim$6 (30fps) days or $\sim$20 days (1fps) of video footage (720p, encoded)~\cite{fortinet-white-paper}. % ~5GB per day
%Even with high-resolution, 4K videos ... ? (need this?)

\paragraph{Network resource is a premium}
As cameras and videos rapidly grow, 
wireless bandwidth scales much slower. 
To stream videos, a camera consumes network bandwidth as high as 1--2 Mbps~\cite{fortinet-white-paper}. 
With cameras deployed on a \textit{shared} network, 
the high bandwidth usage draws users complaints~\cite{complain-camera-1,complain-camera-2}
and researcher attention~\cite{vigil,filterforward}. 
Provisioning \textit{dedicated} network incurs high cost:
the network charge exceeds the camera cost within three months on a Comcast data plan~\cite{Comcast-dataplan}. 
%live streams from 100 cameras would upload 120-400 Mbps would cost more than \$5000 per month per Comcast’s data plan~\cite{Comcast-dataplan}. 
The upcoming 5G is unlikely to eliminate this problem: 
although it promises severalfold bandwidth increase~\cite{huawei-5G}, 
the consumer demand for network bandwidth is projected to grow even faster (e.g., 20$\times$ for VR/AR and 10$\times$ for Internet gaming)~\cite{cisco-white-paper}.
%~\cite{zhang2015design,drone-bandwidth,fortinet-white-paper};
%The network infrastructure (e.g. WiFi) is intended for human users instead of provisioning numerous cameras. 
%After all, in the near future, network bandwidth is likely to remain scarce for inexpensive/numerous IoT cameras.
%Moreover, to enable more accurate analysis~\cite{ruuvzivcka2018fast}, some scenarios even require higher-quality videos to be uploaded, which incurs even more network resource, e.g., 30-40 Mb/s for modern 4K~\cite{filterforward}.
%it does not mitigate the pressure on the last-hop link for numerous wireless cameras.
%it does not mitigate the pressure on the last-hop wireless link. 
%Note that edge compute resources near cameras would help little, 
%as numerous wireless cameras are limited by last-hop wireless bandwidth to reach the edge.

\paragraph{Edge computing is not a silver bullet}
%One may make low-cost cameras stream videos to an edge server. 
To eliminate much the Internet traffic, 
low-cost cameras may stream to edge servers.
However, such connections are typically bottlenecked at the last-hop wireless bandwidth which is in turn limited by precious wireless spectrum today; 
hundreds or thousands of \textit{always-on} video streams will heavily stress the wireless bandwidth.
Furthermore, deploying and managing edge servers may be difficult in remote environments, such as construction sites or offshore oil platforms.

%We design for low-cost cameras. 
%We will examine the applicability to more expensive cameras in evaluation. 

%\subsection{Cold videos are pervasive}
%\subsection{Videos are large and cold}
%A single low-cost camera can produces as much as \Note{20GB} of videos per day. 
%With numerous cameras and ample on-camera storage, 
%a natural implication is that only a small fraction of the captured videos will be eventually queried. 
%This is already observed in existing deployment XXX ... ~\cite{wdblog}.
%The reasons are two. 
%On one hand, as video volume scales, interesting events in video likely remain sparse.
%For example, XXX shows that .... ; XXX shows that ...
%On the other hand, the volume of videos can be produced outstrips compute resource growth;
%\Note{soften this sentence....}
%Analyzing videos is expensive: would require NN accelerators ...
%it takes a \$4,000 GPU to run deep neural networks (NN) with state-of-the-art accuracy over the video stream from a \$25 camera~\cite{noscope,wyzecam}. 

%\subsection{Cold videos are pervasive}
%\subsection{Low-cost cameras incapable ...}
%\subsection{Executing ad-hoc queries}
%\subsection{Executing ad-hoc queries over cold videos}
\subsection{Ad-hoc queries over cold videos}\label{sec:back:evidence}
We support ad-hoc, ``after the fact'' queries~\cite{focus,noscope,vstore}.
%e.g., ``return all frames that contain yellow buses yesterday''.
%They allow queried object classes, expected accuracies, and query operators \Note{parameters?} \notettx{I think the term "parameters" is good here} to be specified by users at query time. 
The query parameters, including object classes, video timespans, and expected accuracies, are specified at query time rather than at video capture time. 
Such queries well suit exploratory analytics,
%as they impose little constraint on user queries flexibility~\cite{eureka,vstore}. 
as they give users high flexibility~\cite{eureka,vstore}. 
%in query semantics and parameters

\paragraph{High-accuracy object detection is essential}
To execute ad-hoc queries, 
object detection is the crucial building block~\cite{blazeit}.
In general, even minor accuracy loss in object detection would incur a substantial loss in overall analytics performance~\cite{gobieski2019intelligence}, for which we further demonstrate in \sect{eval}. 
%While object detection accuracy see significant boost in past years thanks to NN, 
While neural nets significantly advance object detection, 
new models with higher accuracy show unsatisfiable compute demand. 
%especially over real-life videos that could be blurry or non-standard, is far from end yet. 
For instance, compared to YOLOv3 (2018)~\cite{yolov3},
CornerNet (2019)~\cite{cornernet} improves Average Precision by 28\% while being 5$\times$ more expensive.
%CenterNet-HG~\cite{centernet} improves AP by 37\% over YOLOv3 while being 2.56$\times$ more expensive.

%\paragraph{Cameras are incapable of answering the queries by themselves}
%\paragraph{Cameras are incapable of standalone query answering}
%\paragraph{Cameras are incapable of standalone operation}
%\paragraph{Cameras cannot operate alone}
\paragraph{Low-cost cameras cannot answer queries without cloud}
%Low-cost cameras cannot execute video queries with satisfactory accuracy solely by themselves. 
Their CPUs such as Cortex-A53 run state-of-the-art object detection at 0.1 FPS~\cite{nnbenchmarks,yolov2-rpi}, incapable of keeping up with video capture at 1--30 FPS~\cite{focus,noscope}. 
Inexpensive accelerators, while emerging, 
still cannot run high-accuracy object detection fast enough at low enough monetary cost, e.g., Intel's Movidius (\$70) runs YOLOv3 at no faster than 0.5 FPS. 
In the foreseeable future, we expect that the gap between resource demand by high-accuracy object detection and low-cost camera hardware continues to exist. 

%Even with inexpensive accelerators, they still cannot run  high-accuracy object detection in realtime, e.g. Intel's Movidius (\$70) runs YOLOv3 no faster than 0.5 FPS. 

%Beefier accelerators, commonly seen on robots and cameras~\cite{nvidia-jetson-nano} typically cost (2x-3x) of a whole low-cost camera. 
%therefore, these accelerators are commonly seen on robotics or expensive cameras (\textbf{name them??}). 
% ---> and may require active cooling? 

%Second, cost similar or more than an embedded CPU, they add substantially to the bill of materials of a camera. 
%To summarize, 
%the compute need for high-accuracy object detection outpaces the resource of low-cost cameras. 
%In the foreseeable future, we expect the gap to continue to remain. 
%%low-cost NN accelerators are yet to keep up with the growth of object detection compute. 
%%In the foreseeable future, the gap between on-camera NN accuracy and that of the cloud will remain. 
%The implication is that cameras must work with resource-rich cloud (which executes object detectors) to answer queries. 

%\note{Net cameras are increasingly popular, whose traffic is estimated to grow tenfold between 2015 and 2020}~\cite{cisco-visual-networking}


%\subsection{Trends}

% --- useful? ----- 
%As complements, a smaller number of high-end cameras~\cite{jetson-camera} (costing a few hundred dollars), equipped with NPU or GPU~\cite{jetson-tx2-perf}, are deployed strategically in critical locations, e.g., busy intersections.


\paragraph{Cold videos are pervasive}
%\subsection{Videos are large and cold}
%A single low-cost camera can produces as much as 10GB of videos (720p, 1FPS) per day.
With numerous cameras and ample on-camera storage, 
an implication is that only a small fraction of captured videos will be eventually queried, 
as already observed in deployment~\cite{wdblog}.
The reasons are two. 
First, the occurrences of interesting video events remain both unpredictable (thus the need for long-time video capture) and sparse (thus low query rate). 
For example, severe traffic breakdown contributes less than 5\% of the time per day~\cite{trafficpercentage}; 
Foreign Intelligence Surveillance Court only reviewed a tiny fraction of video for terrorism events~\cite{terrorismpercentage}.
Second, analyzing videos is still expensive. 
It would require a GPU of a few thousand dollars to run high-accuracy object detection over video stream from a \$25 camera~\cite{noscope,wyzecam}. 

\input{evidence}

%\paragraph{Low-cost cameras are incapable of answering queries}
\paragraph{The difficulty of streaming}
To analyze videos from cameras, 
many systems follow a ``streaming'' approach~\cite{focus,vstore}: 
%Many prior systems run video analytics over cameras with a ``streaming'' approach~\cite{focus,vstore}: 
%at ingestion time, 
cameras capture and ship videos to the cloud or the edge in real-time, as shown in Figure~\ref{fig:scenario}. 
%\footnote{We do not differentiate them in the paper.}.
While the approach may suit a small number of cameras, each with abundant resources, 
e.g., cameras strategically deployed at busy road intersections, 
%It demands excessive network bandwidth with many low-cost cameras, as described above. 
streaming \textit{cold} videos from \textit{many} low-cost cameras to the cloud is uneconomic. 
To reduce bandwidth usage, recent systems run ``early discarders'' (e.g., motion detection) on camera and only stream surviving videos~\cite{filterforward}. 
Such discarders, however, are effective only when possible queries semantics and parameters are limited and known beforehand. 
To support ad-hoc queries, the discarders to be executed continuously would bloat and become unaffordable to low-cost cameras~\cite{filterforward}.

%When possible queries are diverse (as in many deployment), effective discard operators need to execute common compute for more queries, making them unaffordable to low-end, inexpensive IoT cameras~\cite{filterforward}. 

\begin{comment}
This, however, often faces a dilemma between generality and efficiency: 
to save substantial bandwidth, the early operators must be aggressive. 
When possible queries are diverse, it must be generic and expensive. 
They must be decided in conjunction with queries, which are diverse and may be unknown beforehand, 
the queries are statically baked; 
e.g., a motion detector will not filter more than XXX\% frames from a traffic surveillance camera; 
it works poorly for video that contains lots of motions and for object counting queries. 
it reduces (XX\%) uplink traffic but does not eliminate it. \note{ForwardFilter}
However, generality often comes with higher compute cost, making early discard unaffordable to inexpensive cameras (\$20). 
in particular, models they can run are limited, much lower accuracy, or slow speed. \note{be careful}
\end{comment}



%\subsection{System model}
%\subsection{System model: zero-streaming cameras}
\subsection{System model: zero streaming}
\label{sec:sysmodel}
%Catering to numerous low-cost cameras, 
%Motivated by pervasive low-cost cameras, 
%precious network bandwidth, and cheap on-camera storage, 
%We set to explore an extreme design point, 
%by making the cameras refrain from streaming anything at video capture time. 
We make cameras stream \textit{nothing at all} at video capture time. 
%we advocate for such cameras to refrain from streaming anything at ingestion time: 
%The cameras capture videos to local storage;  
%(where the queries originate) 
Only in response to user queries, 
the cameras collaborate with the cloud to process the queried videos. 
%the cameras communicates with the cloud for processing queried videos. 
%Zero streaming is therefore reactive and efficient: 
Zero streaming caters to limited compute and cold videos: 
%therefore reactive and efficient: 
the system consumes network/cloud resources for only analyzing the queried video, a small fraction of the total captured videos. 

\paragraph{Scope}
%Our goal of querying zero-streaming cameras opens a new design space, in which this paper addresses first-class concerns. 
%Our goal of querying zero-streaming cameras opens a new design space, 
We address the first-class concerns in zero-streaming cameras. 
We focus on cold videos, 
i.e., those queried for the first time. 
We focus on querying individual cameras.
The resultant design serves as the basis for future enhancement, e.g., caching query results for repetitive queries, exploiting past queries for online refinement~\cite{queryrefinement}, and exploiting cross-camera topology~\cite{rexcam}. 
%
We address limited compute resource on cameras~\cite{cheapcam} and limited network bandwidth~\cite{mpdash}. 
We do not consider the cloud as a limiting factor, 
assuming it runs fast enough to process frames uploaded from cameras. 

%\Note{merge this}
%DIVA’s benefit diminishes on repeated queries? 
%Yet, in our target scenario where “cold” videos prevail, repeated queries on given videos are rare.  
%
%We should clarify: ``cold start'' indicates that videos are queried for the first time; it does not refer to the beginning of a query’s execution. DIVA optimizes the whole duration of query execution. 

%As discussed in \sect{intro}, we address challenges from large videos, wimpy cameras~\cite{cheapcam}, and limited network bandwidth~\cite{mpdash}. 
%We do not consider the cloud as a limiting factor, 
%assuming it runs fast enough to process frames uploaded through the bandwidth-limited camera/cloud connection. 


% ----- verbose ----- 
\begin{comment}
%\paragraph{Scope}
%\paragraph{Goals \& Challenges}
\paragraph{Goals \& Scope}
%We target a software system that delivers good performance in querying streamed-nothing cameras. 
%We target a software system that delivers short query delays (hence keeping users in the loop) for streamed-nothing cameras. 
%We target a query execution system for streamed-nothing cameras that delivers short query delays (hence keeping users in the loop). 
We target a software system for querying zero-streaming cameras with interactive performance. 
%hence keeping users in the loop. 
This goal opens a new design space. 
In this paper, we take the initial step and address the first class concerns with minimum assumption. 
Specifically, 
we focus on optimizing individual queries; 
the system performs a ``cold start'' for each query, i.e., no prior knowledge on the queried videos or cameras; 
we focus on querying individual cameras. 
We intend the resultant system to serve as a basis for future enhancement, e.g., exploiting past queries~\cite{queryrefinement} or cross-camera topology~\cite{rexcam}. 
%which we leave as future work. 

%The rationale is that queries are often infrequent~\cite{ihs-report-2016} and the query types can be diverse.
%Assuming no prior knowledge. (cold start) 
%Thus, we design the system for the worst case, always assuming the query never happens before (cold start).
%It does not solve cross camera optimizations. 
%We expect future optimizations are possible and can be stacked atop our design. 

\paragraph{Challenges}
Our goal faces multiple challenges:
one query may cover long video footage in GBs;
cameras have wimpy hardware~\cite{cheapcam} and see limited network bandwidth, typically less than a few MB/s~\cite{mpdash}. 
We do not consider the cloud as a limiting factor, 
assuming it always runs fast enough to process the frames uploaded through the bandwidth-limited camera/cloud connection. 
%by assuming that the cloud always provides sufficient throughput of executing a full-fledged NN over frames uploaded from cameras. 
%This is validated in our evaluation (\S\ref{sec:eval}), showing one modern GPU is capable of supporting queries on 1--2 camera under 1MB/s network bandwidth.
%Besides, it can be easily scaled up with more GPUs with modest cost as it is on-demand.
Towards these challenges, prior video systems are inadequate: 
as discussed in \sect{intro}, they either optimize for live analytics~\cite{lavea,filterforward} 
or rely on heavyweight ingestion~\cite{focus} that mismatches 
resource-constrained cameras. 
We will present evidence in \sect{eval}.
\end{comment}


==> recycle/recycle-eval.tex <==
% !TeX root = main.tex

\section{Evaluation}
\label{sec:eval}

%We evaluate \sys{}'s overall performance (\S\ref{sec:eval:e2e}) and how much do the key designs matter (\S\ref{sec:eval:exec} \& \S\ref{sec:eval:lm}).

We evaluate the overall performance (\S\ref{sec:eval:e2e}) and the key designs (\S\ref{sec:eval:exec} \& \S\ref{sec:eval:lm}) of \sys.

%We seek to answer the following questions: 
%\begin{myitemize}
%\item \S\ref{sec:eval:e2e}: Does \sys{} achieve good performance? 
%\item \S\ref{sec:eval:exec} \& \S\ref{sec:eval:lm}: How much do \sys{}'s key designs matter? 
%%\item \S\ref{sec:eval:adapt}: Does \sys{} adapt to different hardware resources? 
%\end{myitemize}

\input{eval-method}
\input{eval-perf}
\input{eval-comp}
\input{eval-local}
%\input{eval-adapt} %--- xzl: useful but verbose; may resurrect
% \input{eval-train}
% \input{eval-scale}

==> recycle/recycle-intro.tex <==
% !TeX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% xzl: This is the Intro. It can be produced as part of the paper PDF and a standalone html.
% -- Don't put any non standard latex commands here. No need to save space.
% 
% html: see summary/
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \newcommand{\isolation}{Enforcing isolation with ARM TrustZone}
%\newcommand{\noconcurrency}{Stay oblivious to concurrency management}
% \newcommand{\noconcurrency}{Exposing low-level abstractions of trusted computations}
%\newcommand{\seqmm}{Unbounded arrays as the primary data structure}
% \newcommand{\seqmm}{Unbounded arrays as the universal memory abstraction}
% \newcommand{\hints}{Exploiting performance hints from the untrusted}

\section{Introduction}
\label{sec:intro}


%Surveillance cameras see 140M annual shipment~\cite{ihs-report-2018}. 
Surveillance cameras are pervasive: 
many organizations run more than 200 cameras 24$\times$7~\cite{seagatereport}.
They produce videos with high business/social values, which can be extracted by queries such as 
``get the daily peak pedestrian count in the past week''~\cite{lipton2015video,zhu2017online,shi2018geometry,beymer1997real}. 
%``get video frames from yesterday that contain yellow buses''. 
%e.g., for theft investigation, wildlife study, and traffic planning. 
%Three notable trends motivate our work. \Note{insights, observations...?}
%Three key observations of recent trends motivate our work.
Three trends motivate our work.

%\paragraph{Low-cost cameras in mass development}
%\paragraph{Fast growth of low-cost cameras}
\noindent 
%\textit{(1) The fast growth of low-cost wireless cameras} \hspace{1mm}
\textit{(1) Low-cost, wireless cameras grow fast}
\hspace{1mm}
As key complements to high-end cameras, 
low-cost cameras (<\$40) are increasingly pervasive~\cite{wyze-camv2,yi-cam,zosi-cam}. 
% --- useful, but .5M shipment does not sound a lot ---- 
%For instance, WyzeCam (\$25) ships more than half a million units annually~\cite{wyzecam-success}.
These cameras often have limited compute resource yet spacious storage (see \sect{bkgnd}). 
Being wireless, these cameras are meant to be installed by individuals or small businesses with ease just as other wireless sensors~\cite{install-humidity-sensor}.
%Complementing a smaller number of high-end cameras, 
%numerous low-cost cameras will offer pervasive coverage of urban and rural areas.  

%Retrospective analytics is efficient for harnessing colossal surveillance videos, of which only a small fraction \note{check}~\cite{wdblog} will be eventually queried~\cite{ihs-report-2018}. 

%\paragraph{Most videos are cold} 
\noindent \textit{(2) Most videos are cold} \hspace{1mm}
\begin{comment}
%\st{A single camera produces as many as 24GB video per day}~\cite{vstore}. 
As the focus of this work, ``after-the-fact'' query contains parameters that cannot be foreseen, e.g., queried range and object.
Those queries are issued in low frequency, typically after an interesting but rare event happens, e.g., criminal or stealing.
As a result,
most captured videos will never be queried~\cite{wdblog}.
The situation is getting amplified by the fact of ever-increasing installed cameras~\cite{wyzecam-success} and expensive video analytics~\cite{centernet}.
%With fast growth of cameras, 
%This is because interesting video events remain sparse and video analytics is in general compute-expensive~\cite{noscope,wyzecam}.
%For example, security cameras installed in a retail store may only be queried after stealing happens, which is very rare event.
\end{comment}
%In many key scenarios, 
Users typically deploy cameras for capturing \textit{excessive} videos, despite knowing most of the captured videos will never be queried~\cite{wdblog}.
The reason is fundamental: 
interesting video events are often rare and unforeseeable; 
the need for examining such events emerges well after video capture~\cite{eva}.
For instance, one may investigate a \textit{past} store theft by querying videos captured nearby. 
Furthermore, the compute cost of video analytics is still high~\cite{focus,noscope}, dwindling the fraction of captured videos can be analyzed. 
\sect{bkgnd} will provide evidences for cold videos.

%several to tens of GB per day~\cite{cisco-white-paper}. 


\input{tab-scenario}

%\paragraph{Network resource is a premium} 
\noindent \textit{(3) Network resource is a premium} \hspace{1mm}
Wireless bandwidth grows much slower than the volume of captured videos. 
If streaming video in real-time, a camera consumes network bandwidth as high as 0.1--0.2 MB/s, 
which will be further multiplied by the large number of cameras.

\mwx{
On shared WiFi which provides only 0.2 -- 3.3MB/s across different countries according to a global measurement in late of 2018~\cite{wifi-state} and also academia findings~\cite{mpdash}, 
}
streaming cameras inflict poor user experience~\cite{complain-camera-1,complain-camera-2}. 
On a dedicated up link, streaming cameras incur substantial monetary cost of  network traffic, which exceeds the cost of camera hardware in three months~\cite{Comcast-dataplan}. 
Although 5G promises severalfold bandwidth increase, 
the consumer demand is projected to grow even faster~\cite{huawei-5G}.
In short, provisioning network for streaming \textit{cold} videos is uneconomic, if ever feasible. 
%\note{yunxin: how about WiFi?}

% --- verbose ---
\begin{comment}
We assume (ad hoc), generic queries: user may query any object class recognizable by modern NN, e.g. 80 classes of YoloV3. 
The queried class cannot be foreseen at ingestion time. 
We target three types of queries: 
\textit{Retrieval}, e.g., ``returning video frames containing buses yesterday'';
\textit{Tagging}, e.g., ``returning time ranges when deers show up'';
and \textit{Counting}, e.g., ``return the median of pedestrian count during day time''. 
They cover a wide range of video analytics scenarios, e.g. for transportation traffic and wildlife (smart retailing?) \note{cite}.
\note{They can also serve as building blocks of more advanced and complicated query types.}
\end{comment}




%While recognizing the design space is large and many intermediate points (various discard operators, various camera hardware capabilities) are possible, 

%\paragraph{Streamed-nothing cameras}
%\paragraph{Zero-streaming, low-cost cameras}
%\paragraph{Implication: zero streaming}
\paragraph{Zero streaming \& its use cases}
%How to analyze large, cold videos that are continuously produced by many low-cost cameras?
How to analyze large, cold videos produced by many low-cost cameras?
We advocate for a system model dubbed ``zero streaming''. 
%as shown in Figure~\ref{fig:overview}.
(1) Cameras continuously capture videos to their cheap local storage without uploading any. 
(2) Only in response to a retrospective query, 
%e.g., ``return all frames containing yellow buses yesterday'', 
the cloud reaches out to the queried camera, coordinating with it to process
the queried video. 
%\st{Optionally, cameras may periodically present proof of video possession to the cloud.}
(3) While the video is being processed, the system presents users with inexact yet useful results and continuously refines the results until query completion~\cite{ola}. 
A user may \textit{explore} videos through interactive queries, e.g. aborting an ongoing query based on early results and issuing a new query with revised parameters~\cite{eva,eureka}.
%This supports users to interactively \textit{explore} videos: 
%they repetitively try queries; 
%based on partial results, they abort an ongoing query and issue a revised query~\cite{eva,eureka}. 
%By querying zero streaming cameras, 
%Through exploratory queries over zero streaming cameras,
%A variety of applications can be built, for example: 
%Zero streaming cameras support a variety of use cases:
The system model supports rich use cases, for example:

\begin{myitemize}
\item 
To investigate a theft, a manager queries the cameras in and out of a warehouse, requesting video frames containing persons matching certain descriptions.
\item 
To understand how recent visitors impact bobcat activities, a ranger queries all the park's cameras, requesting time ranges where the cameras capture bobcats.
%for wildlife monitoring, zookeepers monitor how long does an elephant stay aside the river each day;
\item 
To trace the cause of recent frequent congestion on a high way, 
a city planner queries cameras on nearby local roads, requesting car counts seen on these local roads.
\end{myitemize}

Zero streaming suits low-cost cameras in large deployment. 
At video capture time, the cameras are highly resource-conserving, 
requiring no network or external compute resource such as cloud GPU instances.
The cameras can thus operate on constrained or on-demand networks, e.g. long-range wireless~\cite{lora}.
Only to process a query, the deployment requires network and external compute resources. 


\begin{comment}
%Exploratory analytics over zero-streaming cameras
%The system model 
Zero streaming suits low-cost cameras in large deployment. 
%Most video analytics activities shift from video capture time to query execution time. 
%Most compute and activities happen at query execution time rather than video capture time. 
As a result, the cameras require no network bandwidth for video capture, 
capable of operating on constrained or on-demand networks, e.g. long-range wireless~\cite{lora}.
%The ingestion uses zero network bandwidth and only uses network bandwidth. 
%making large camera deployment under limited network bandwidth possible. 
%This scales well with a larger number of cameras  (hundreds or thousands). 
%Such cameras particularly suit deployment in remote areas, where network may be provisioned on-demand through long-range wireless~\cite{lora}.
The whole camera deployment incurs low compute cost: 
%it only requires constrained camera hardware 
video capture is completely executed on cameras; 
cloud resources (e.g. GPU instances) are only needed at query time. 
\end{comment}

Zero streaming adds a new point to the space of video analytics, as shown in Figure~\ref{fig:scenario}. 
It facilitates retrospective, exploratory analytics, a key complement to other analytics, including real-time event detection and low-delay video retrieval. 
The latter analytics often demands much higher compute/network resource per-camera and hence
only suit a small number of cameras deployed on critical locations, e.g., busy road intersections~\cite{videostorm} \Note{why cite this?}.

%cite ~\cite{cheapcam,wyzecam}  ??

%cameras with constrained hardware will suffice and cloud resource is only needed at query time. % but never for ingestion. 
%resonating well with the cloud's on-demand spirit. 
%The billing model is clean: charging the resultant cloud usage to whoever queries. 

%It is worth noting that: we expect that \sysmodel{} complement to, but not substitute for, live video analytics; 
%Despite resource efficient, zero-streaming cameras supports \textit{exploration} of large videos, as we will show in the paper. 
%We focus on support \textit{exploratory analytics} of large videos stored on zero-streaming cameras,
%where revise, refine queries...\cite{eva}

%A variety of attractive applications can be built on 
%retrospective queries over cold videos stored on zero-streaming cameras, for example:
%Through retrospective queries over cold videos stored on cameras, 
%a variety of applications can be built, for example: 
%Through querying cold videos stored on many low-cost cameras, 


%By doing so, zero-streaming cameras support \textit{exploration} of videos stored on the cameras
%We focus on supporting users to \textit{explore} videos on zero-streaming cameras:
%despite running a query to its completion take 
%a user sees inexact query results as soon as she starts the query; 
%based on the results, she may abort the query, revise the parameters, and issue anew \cite{eva,eureka}. 

%Note that we do not expect zero streaming to substitute for the streaming approach, 
%which uploads videos for live analytics or real-time archiving. 
%With much higher resource consumption per-camera, the approach suits a small number of cameras that are strategically deployed on critical locations, e.g. busy road intersections.
%\Note{integrate this better}

%while capturing videos (ingestion time), a camera keeps storing video footage on local storage without uploading any data;
%it remains completely radio silence; 

%Our approach is motivated by cheap on-camera storage:
%Inexpensive cameras are already capable of storing days/weeks of videos. 
% -- on-camera storage is cheap. A 64GB uSD card costs XXX \$ which can store XX days of 720p videos (typically lifespan). 

% ---- verbose ---- 
\begin{comment}
This results in efficient, on-demand use of compute infrastructure, specifically:
\begin{myitemize}
\item 
Network bandwidth is only used by queries but never by ingestion, 
making large camera deployment friendly to limited network bandwidth. 
%The ingestion uses zero network bandwidth and only uses network bandwidth. 
%making large camera deployment under limited network bandwidth possible. 
%This scales well with a larger number of cameras  (hundreds or thousands). 
Zero streaming further suits cameras deployed in remote areas, for which long-range network connectivity, e.g., LoRa~\cite{lora}, only has to be provisioned at query time, e.g., from drones.
\item 
Cloud compute resources is only needed for query but never for ingestion. 
This resonates with cloud's on-demand spirit and results in a clean billing model: 
charging cloud usage to users whoever query. 
\end{myitemize}
\end{comment}

%\paragraph{Challenges}
%Can we build a query processing system for \sysmodel{} to provide interactive performance
%and uncompromised accuracy?
%Can \sysmodel{} answer queries with interactive performance and uncompromised accuracy?
%With zero streaming, 
%Can we query videos stored on low-cost cameras with interactive performance and uncompromised accuracy?
%On one hand, a query may concern GBs of on-camera video that spans days. 
%On the other hand, 
%low-cost cameras often have low-end CPUs~\cite{cheapcam,wyzecam}; 
%their uplink bandwidth is often no more than a few MB/s~\cite{mpdash}. 

%Existing video analytics systems are inadequate in addressing these challenges. 
%To query \sysmodel{}s, 

\paragraph{\sys{}}
To support querying zero-streaming cameras, 
we present a camera/cloud runtime system called \sys{}. 
As shown in Figure~\ref{fig:overview},
a camera captures video to local storage. 
In response to a query, the camera works in conjunction with the cloud:
the camera runs operators, implemented as lightweight neural nets (NNs), to \textit{rank} or \textit{filter} frames; 
the cloud runs full-fledged object detection to validate results uploaded from the camera.  

%\paragraph{Challenges \& solutions}
The central challenges to \sys{} are two. 
%We identify two central design questions. 
%First, (ingestion time indexing??) 
%during video capture, 
%%how should the system best use limited on-camera resource 
%what computations should the system run on camera 
%in order to speed up forthcoming queries? 
%(1) During video capture: how should the system best use on-camera resources to optimize forthcoming queries? 
(1) During video capture: how should cameras best use their limited resources to optimize future queries? 
%Second, (query planning??) 
%during a query, how should the system schedule 
%numerous video frames for processing and schedule the results for delivery?
%Second, 
%to execute a query, how should the system discover the most promising query results, by orchestrating on-camera computation with network transmission and prioritizing numerous video frames?
%(2) To execute a query: how should the system orchestrate on-camera computation and network transmission, both seeing tight resource constraints, to discover and deliver useful query results to the user as soon as possible?
(2) To execute a query: how should the cloud and the camera orchestrate, in order to deliver useful query results to the user as soon as possible?
%
%during a query, how should the system schedule its limited compute and network resources? In particular, the system should 
%prioritize numerous video frames for processing and prioritize the results for delivery 
%
Existing techniques are inadequate.
Recent video systems pre-process (``index'') video frames as capturing them~\cite{focus}
and answer queries based on indexes only. 
%when a query comes in, the system speeds up execution by only processing the built indexes. 
%Such a design mismatches low-cost cameras, which 
%they can only afford to build low-accuracy indexes, resulting in poor query performance.
%are incapable of building accurate indexes in real-time and hence answer queries poorly.
Yet, low-cost cameras cannot build indexes usable to queries in real-time.
Many systems process video frames in a streaming fashion~\cite{vigil,lavea,filterforward}. 
While suitable to live videos as shown in Figure~\ref{fig:scenario}, they would miss key objectives in retrospective queries, e.g. fast discovery of useful results. 
%e.g., prioritizing frames or processing frames in multiple passes. 
%e.g. processing the queried frames in multiple iterations.
%strategically sampling all queried frames or prioritizing their processing. 
%Recent proposal on partitioning computation between ingestion time (building \textit{inexact}, real-time indexes) and query time (processing the indexes)~\cite{focus} is also suboptimal: 
%Recent systems propose to split video analytics workloads between ingestion time and query time: 
%the ingestion indexes all input frames with object detection, so that the query executor only needs to process the indexes at low cost~\cite{focus}. 
We will demonstrate the inadequacies in \sect{eval}. 
%experimentally (\S\ref{sec:eval}). 

\input{fig-overview}

%We build \sys{}, an analytics engine for querying videos stored on low-cost surveillance cameras, as shown in Figure~\ref{fig:overview}.
%\notettx{In response, we build \sys{}, a fully automatic analytics engine for querying videos stored on low-cost surveillance cameras, as shown in Figure xxx. Specifically, \sys{} opens a new design space for ``first-time'' queries given that only a small fraction of the video will be eventually queried (cite xxx), i.e., most data are "cold".}
%We build \sys{}, 
%a runtime system for \sysmodel{} to answer retrospective queries, 
%as shown in Figure~\ref{fig:overview}. 
%Our runtime system called \sys{} is shown in Figure~\ref{fig:overview}. 
%In a nutshell, 
%As continuously capturing video footage, 
%during video capture, a camera stores all video frames and samples frames for processing. 
%the camera runs lightweight operators, i.e. frame rankers and filters implemented as neural nets, on cameras and a full-fledged object detector in the cloud in conjunction; 
%\st{the cloud validates results uploaded from the cameras or processes frames undecidable to cameras.}
%With \sys{}, a camera continuously captures video and processes a small sample of the video frames. 


%or processes frames undecidable to cameras.}
%Since full query execution is slow (large data and constrained camera resources), 
%In the face of large data and wimpy camera hardware, 
%\sys{} embraces online query processing~\cite{ola}:
%it delivers partial or inexact results to users as soon as a query starts and continuously refines the results until query completion.
To this end, \sys{} has two unconventional designs. 
%Similar to prior systems~\cite{noscope}, 

%Unlike many prior systems, it does Generic queries. Can query many object classes (e.g. those defined in XXX). does not assume a small set. 
%In a nutshell, \sys{} consists of a (simple) camera runtime and a cloud query engine. 
%The camera runtime continuously processes videos at ingestion; 
%in response to a user query, the cloud engine plans query execution, spreading it over the camera and the cloud: 
%the cloud engine bootstrap simple operators specialized for the query and the queried video; 


\begin{myitemize}
\item 
%\textbf{Ingestion: slow but sure}: 
%\textbf{Capture time: building sparse but sure landmarks} 
\textbf{During video capture: building sparse but sure landmarks 
for distilling long-time knowledge}
(Figure~\ref{fig:overview}(a); $\S$\ref{sec:lm}) 
%As the camera continuously ingests and stores videos, 
On a small sample of captured video frames dubbed \textit{landmarks}, 
the camera runs generic, expensive object detection, e.g., the YOLOv3 NN~\cite{yolov3}. 
This is opposite to existing designs: detecting objects with low accuracy on all/most frames as capturing them~\cite{focus,filterforward}. 
%Limited by on-camera resources, landmarks are sparse, e.g. one in every 30 captured frames;
%Constrained by resources, 
%With limited resources, cameras can only generate sparse landmarks, e.g. one in every 30 captured frames;
Constrained by the camera hardware, landmarks are sparse in time, e.g., one in every 30 captured frames;
yet, with high-accuracy object labels, they provide \textit{reliable} knowledge 
-- spatial/temporal distributions of various objects over long-term videos.
%\sys{} does not use the sparse landmarks to directly answer queries but builds key query optimizations atop them. 
%\sys{} does not use the knowledge as direct answers to queries but as basis for key query optimizations. 
\sys{} does not use landmarks as direct answers to queries but as basis for optimizing queries. 
%Spread over long videos, 
Specifically, 
\sys{} guides its query execution with long-term object skewness learned from landmarks and
bootstraps operators by using landmarks as training samples.
%and uses landmarks as initial answers to queries.
%These would be impossible with the common design that runs low-accuracy object detection on all/most frames~\cite{focus,filterforward}, as we will show experimentally in \S\ref{sec:eval}. 



%(with detected objects) yield key long-term distribution of objects for optimizing query operators, e.g. ``95\% bus instances appear on the bottom right region of video frames''; 
 

 
\item 
%\textbf{Query time: iterative execution with (XXX automatic?? in-query XXX) operator upgrade}
%\textbf{Query time: iterative execution with in-query operator upgrade}
%\textbf{Query time: iterative execution with operator upgrade}
%\textbf{Query time: multipass processing with online operator upgrade}
\textbf{To execute queries: multipass processing with online operator upgrade}
(Figure~\ref{fig:overview}(b); $\S$\ref{sec:op}) 
For one query, 
the cloud trains a family of operators with diverse accuracies/costs. 
Throughout the query execution, the cloud keeps pushing new operators to the camera, picking the next operator to push based on query progress, network conditions, 
and operator accuracies. 
%The cloud not only specializes the operators for the queried video, 
%but also picks the next operator to push 
%but also keeps pushing the next operator for the camera to run picked based on query progress, network/camera resources, and the outcome of online operator training \Note{what does this mean}.  
%and the observed resources (network bandwdith and camera speed). 
%With the operators, 
The camera processes video frames in multiple passes, one pass with an operator.
The early operators quickly \textit{explore} the frames for inexact answers 
while the later operators slowly \textit{exploit} for more exact answers. 
This contrasts to prior systems that process queried frames in one pass, with operators determined ahead of the query~\cite{noscope,filterforward,blazeit}.

\end{myitemize}

%\Note{highlight users do not have to involve. fully automatic.}

%\notettx{\textbf{Users can be totally ``hands-off''}}
%\notettx{\sys{} is designed as a fully automatic analytics engine, which means that users do not have to involve in the query loop. However, we reserve the possibility that the user is satisfied with the partial results and early abort the query.} 

% --- good but verbose --- 
%Beyond the two designs, \sys{} further employs important optimizations, 
%including operator training at query time, scheduling frames for processing, and tracking optical flows. 

Evaluated with 720-hour videos from 15 different scenes,  \sys{} runs queries at more than 100$\times$ video realtime on average, with typical wireless conditions and low-cost embedded hardware.
\sys{} returns partial results quickly: 
compared to executing a query to completion, 
\sys{} only spends 12\% of the time to return 50\% of all the frames of interest, 
resulting in 1,070$\times$ video realtime. 
%e.g. in the first 1/10 period of a query's total execution, it returns 50\% of the needed video frames, 
%resulting in a XXXx video time. 
Compared to competitive alternatives, \sys{} speeds up queries by at least 4$\times$.

\begin{comment}
\sys{} spends as low as 2.1 minutes (18 minutes in average) to \textbf{fully} execute query over 48-hour videos, or 1370$\times$ realtime speedup. 
To return 50\% of query results, it takes as low as 75 seconds (2300$\times$ realtime).
Furthermore, \sys{} is robust in extreme condition like wimpy hardware platforms and limited bandwidth, in which the benefit only goes down by XX$\times$ and XX$\times$, respectively.
We will show more thorough results in Section \mbox{\ref{sec:eval}}

\sys{} spends 23 minutes in average (2.1 minutes in best case) to \textbf{fully} execute query over 48-hour videos, or 125$\times$ realtime speedup. 
To return 50\% of query results, it takes only 2.7 minutes in average (1,070$\times$ realtime).


\end{comment}




\paragraph{Contributions}
We have made the following contributions. 
\begin{myitemize}

\item Zero streaming,  a new model for low-cost cameras to operate on frugal network while answering video queries.  

\item Two unconventional ideas for querying zero-streaming cameras:
%landmarks for 
capturing accurate knowledge from sparse frame samples rather than inaccurate knowledge on all frames; 
%online operator upgrade for 
processing frames in multiple passes with operators continuously picked during a query, rather than one-pass processing with operators decided ahead of a query. % ahead of time.
%for video ingestion time and operator upgrade for query time. 

\item \sys{}, a concrete implementation that runs queries at more than 100$\times$ realtime with uncompromised query accuracy.
%a video query processing system that instantiates the designs. 
%Evaluated on large video datasets, \sys{} runs queries at more than 100$\times$ video realtime with uncompromised query accuracy.
%significantly outperforms competitive alternatives.
\end{myitemize}


To our knowledge, \sys{} is the first system designed for querying large videos stored on low-cost remote cameras. 


==> tab-design.tex <==
% !TeX root = main.tex

\begin{table}[]
\small
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{design} & Where's video & \textbf{Ingestion} & \textbf{Query} \\ \hline
NoScope &  cloud & -- & One specialized op per video \\ \hline
Focus & cloud & Approximate all frames & Index processing \\ \hline
Vigil & wireless cam  & ?? simple/fixed op & ?? \\ \hline
\sys{} & wireless cams & Slow sure generic op & Multipass specialized op \\ \hline
\end{tabular}
	\caption{A comparison vs. related video analytics \textbf{Vigil may be removed}}
\label{tab:design}
\end{table}

==> tab-exp.tex <==
% !TeX root = main.tex

\begin{table}[]
\scriptsize
\begin{tabular}{l|l|l|c}
\hline
\textbf{} & \textbf{Cam:Capture} & \textbf{Cam:Query} & \textbf{Cloud:Query} \\ 
\hline
ClondOnly 	& -- & Only upload frames &  \\ 
OptOp  	& Yv3 every 30 frames & Run one optimal op & Yv3 on all \\ 
PreIndexAll & YTiny on all frames & Parse YTiny result & uploaded frames \\ 
\sys{}    & Yv3 every 30 frames & Multi passes \& ops &  \\ \hline
\end{tabular}
\vspace{0.3cm}
	\caption{
	\textbf{\sys{} and the alternatives in test}. The table summarizes their executions for capture and query. 
	NN models: Yv3: YOLOv3, high accuracy (mAP=57.9 on COCO dataset);
	YTiny: YOLOv3-tiny, fast and low accuracy (mAP=33.1). 
	%Both are state of the art.
	}
\label{tab:exp}
\end{table}

%  Mengwei's
%
%\begin{tabular}{|l|l|l|l|l|}
%\hline
%\textbf{} & \textbf{Ingest/Cam} & \textbf{Query/Cam} & Query/Cloud \\ 
%ClondOnly 	& -- & Upload frames only & \multirow{4}{*}{Yv3 on all} \\ \cline{1-3}
%OptOp  	& Yv3 every 30 secs & One optimal op &  \\ \cline{1-3}
%PreIndexAll & YTiny on all & Process YTiny result &  \\ \cline{1-3}
%\sys{}    & YTiny every 30 secs & Multi ops &  \\ \hline
%\end{tabular}

==> tab-perfvscost.tex <==
\begin{table}[]
\small
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{platform} & \textbf{fps} & \textbf{price (\$)} & \textbf{fps per dollar} \\ \hline
raspberry pi 3 & 2 & 35 & 0.06 \\ \hline
%https://github.com/samjabrahams/tensorflow-on-raspberry-pi/tree/master/benchmarks/inceptionv3
neural compute stick & 3 & 70 & 0.04 \\ \hline
ROCK 960 & 24 & 100 & 0.24 \\ \hline
%https://www.cnx-software.com/2018/01/08/rockchip-rk3399pro-soc-integrates-a-2-4-tops-neural-network-processing-unit-for-artificial-intelligence-applications/
HiKey 970 & 18 & 300 & 0.06 \\ \hline
Jetson TX2 & 20 & 500 & 0.04 \\ \hline
\end{tabular}
\end{table}

==> tagging_algo.tex <==
% !TeX root = main.tex


%\vspace{-5pt}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\begin{algorithm}
	
\footnotesize
\caption{frame scheduling for each tagging pass}\label{algo:tagging}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{$op$: operator $group\_size$: (30, ... 1) \\
$P, N, U$: pos/neg/undecidable tags\\
}
\Output{$P, N, U$ (updated)}

$Q$ $\gets$ initialize upload queue\\
%$groups$ $\gets$ divide the query time range into groups based on $window\_size$\\
$groups$ $\gets$ divide the query time range into groups \\
\For(\tcp*[h]{rapid attempting}){$g$ in $groups$}{
	\lIf{any frame in $g$ is $P$/$N$}{
		pass
	}
	\lElseIf{any frame in $g$ is $U$}{
		add frame to $Q$
	}
	\uElse{
		$f$ $\gets$ pick a random frame from $g$\\
		process and tag $f$ with $op$\\
		\lIf{$f$ tagged as $U$}{
			add $f$ to $Q$
		}
	}
}
\While(\tcp*[h]{work stealing}){$Q$ is not empty}{
	$f \gets Q$.tail(); $g$ $\gets$ enclosing group of $f$ \\
	$f1$ $\gets$ an untagged frame within $g$ \\
	process and tag $f1$ with $op$ \\
	\lIf{$f1$ tagged as $P$/$N$}{
		remove $f$ from $Q$
	}
}
%\notettx{use even smaller fonts? like footnotesize}
\end{algorithm}
%\vspace{-10pt}

==> tagging_algo_old.tex <==
\algdef{SE}[VARIABLES]{Variables}{EndVariables}
   {\algorithmicvariables}
   {\algorithmicend\ \algorithmicvariables}
\algnewcommand{\algorithmicvariables}{\textbf{global variables}}

\algtext*{EndWhile}% Remove "end while" text
\algtext*{EndIf}% Remove "end if" text

\begin{algorithm}
\caption{on-camera tagging algorithm for one epoch}
\small
\begin{algorithmic}[1]

\Variables
 \State $Q$: uploadng queue
 \State $P, N, U$: positive, negative, and uncertain frames that have been tagged by on-camera operator or cloud oracle
\EndVariables

\Procedure{Scanning}{$op, G$}
%	\State scanning each frame in group $G$:
	\If{at least one frame in $G$ is $P$/$N$} \Comment{already resolved}
	\State return
	\ElsIf{at least one frame in $G$ is $U$} \Comment{tried in last epoch}
	\State add this frame to $Q$, return
	\Else \Comment{no frames have been processed}
	\State $F$ $\gets$ pick a random frame from $G$
	\State process and tag F with $op$
	\If{$F$ tagged as $U$}
	\State add $F$ to $Q$
	\EndIf
	\EndIf	
\EndProcedure

\Procedure{Revisiting}{$op$}
    \For{$F \gets Q$\_tail to $Q$\_head}
    \State $G$ $\gets$ enclosing group of $F$
    \State $F1$ $\gets$ an untagged frame within $G$
    \State process and tag $F1$ with $op$
    \If{$F1$ tagged as $P$/$N$}
    \State remove $F$ from $Q$
    \EndIf
    \EndFor
\EndProcedure

\Procedure{tagging}{$op$, $refinement$}
	\State $groups$ $\gets$ divide the query time range into groups based on the refinement level
	\For{$G$ in $groups$}
	\State $\textsc{Scanning}(G)$
	\EndFor
    \While{$Q$ is not empty}
        \State $\textsc{Revisiting}(op)$
    \EndWhile
\EndProcedure

\end{algorithmic}\label{algo:tagging}
\end{algorithm}

==> training.tex <==
% !TeX root = main.tex
%\subsection{Just-in-time Training Shallow NNs}
%\subsection{A Factory of on-camera operators (?)}
\section{the operator factory (?)}

\note{much of the contents may go to a later section?}

\noindent \textbf{Just-in-time training (bootstrapping)}: the shallow NNs will be trained at query time, 

\note{one factory instance for each time-range (e.g. 6 hours of videos?)}

\note{What's new?}\note{Key idea}: 
discovering training samples?
training happens in parallel to query? 

\textbf{the factory's interface}: 

\begin{myitemize}
\item training samples and the queried object class. 
\item output: a portofolio of models. (including crop regions, resolution, etc). each model has accuracy and speed. 
The accuracy comes from the training/testing. 
The speed comes from the camera's hardware model. 
\end{myitemize}

\noindent \textbf{Candidates}: list of compressed versions of AlexNet.
\begin{itemize}
\item \textbf{Speed-accuracy trades-off}: different resize ratio, convolutional layer number, kernel sizes, and dense size.
\item \textbf{Heatmap-based cropping}: shallow NNs are trained on cropped regions.
\item \textbf{Time-window-based customization}: one generic shallow NN will be trained for the whole time range being queried, then customized for each time ranges.
\item MOVED \textbf{Controlling positive ratio of training samples}: using optical flow.
(From Mengwei)
our query might target at infrequent objects, e.g., only 1\%. randomly sending frames to train doesn't work well, as ML community demonstrates that (I guess so) we need certain pos ratio to train a good bin classifier. Straightforward approach is just sending more frames and we can downsample the negative frames. Since we have optical flow, we are able to collect more positive frames, thus training better NNs or fewer frames to send.

\end{itemize}

\textbf{How to crop based on heatmap}? We will crop at a set of fixed level (99\% instances, 90\% instances, ...)
Should we choose so based on the queries as well? No?

\textbf{Natural question:} is training time a problem? No because bin ops are in general small. 

The training does not end in one shot; it goes on throughout the entire (most of?) query process. 
The small ops require fewer training samples; when its accuracy stablizes, the system can use it. 
Meanwhile, as the query continues, the cloud (factory) keeps receiving more frames (retrieval, counting) as training samples. The factory keeps trains the ops. This helps further imrpove the accuracy of large models (tens of K frames?). 

\textbf{how to decide when to ship out initial bin op?}
\begin{myitemize}
\item collect LMs \& adjacent frames. Send bin op when small bin ops accuracy start to stablize. (?)
\item Okay to ship out even when small binop accurcy still goes up (I guess no beacuse we only need a few K?)
\item What if still no enough training samples? Generic model?
\end{myitemize}


\paragraph{time-range of ops}
Similarly, we want to minimize the knowledge needed to be learnt by our shallow NNs. As observed, the video contents can change dramatically because of weather condition, light condition, etc. By observing the videos, we can roughly divide a long-range video into different sub-videos, each of which has relaltively stable contents.
\textbf{how to choose the time range length? to discuss in impl?}

\textbf{Manufacturing - one time for each query} 
a list of shallow NNs with trades-off between accuracy and speed based on the training samples, cropping regions, time windows. Candidates are a list of compressed version of AlexNet. 
\textbf{talk about the net arch in implementation)}
We can say something like selecting candidates to cater into the input information, but doesn't help much as bin ops training is not the bottleneck here. 

\textbf{Because bin ops are in general simple, each operator's training time is seconds, which is short compared to query execution}

%\item \textbf{Selecting}: 
\textbf{Shopping - repeated multiple times per query}: 
we expose the following abstraction. 
\note{the unified abstraction and interface} 
speed and accuracy
Often the selection as a maxmin condition, e.g. 
For instance, it could be ``among all ops with speed highest than $P$, return the one with the highest accuracy''. 


\note{need thoughts and good writing.}
basically shallow NN is a ``factory'' -- produce NNs on demand catering to the execution plan. What are the parameters for NNs? 








\note{what are the objectives we tradeff? eg} camera speed, accuracy. network bw. 


\paragraph{Discovering training samples}
\st{Controlling positive ratio of training samples}: using optical flow.
(From Mengwei)
our query might target at infrequent objects, e.g., only 1\%. randomly sending frames to train doesn't work well, as ML community demonstrates that (I guess so) we need certain pos ratio to train a good bin classifier. Straightforward approach is just sending more frames and we can downsample the negative frames. 
This ``uniform'' sampling was done in prior work~\cite{noscope} which assumes training samples are ample. 
Since we have optical flow, we are able to collect more positive frames, thus training better NNs or fewer frames to send.
\note{opflow can go to a later section. Can we show that w/o opflow, how bad it could be?}


\noindent \textbf{Overhead of sending training samples}: not much.
\begin{itemize}
\item The shallow NNs are small (few params), so the number of samples needed to train them is small. Typically several K is enough.
\item Because the landmarks are already tagged by local oracle model, we can send the frames with low resolution (highest input size of all candidates, e.g., 100X100).
\end{itemize}

\paragraph{Training larger models}
Different models require different numbers of training samples. Small model only require several K, so landmarks are enough. But big model need more than landmarks, so it fits into our interactive design, since we always use a small model first, but keep sending frames (in each query pattern) so we can train a better one for later stage.

\textbf{It would be neverthless important to show that we can bootstrap when training samples are insufficient}
Not our contribution. But should show it can work. 
